ChainedFilter: Combining Membership Filters by Chain Rule

Membership (membership query / membership testing) is a fundamental problem across databases, networks and security. However, previous research has primarily focused on either approximate solutions, such as Bloom Filters, or exact methods, like perfect hashing and dictionaries, without attempting to develop a an integral theory. In this paper, we propose a unified and complete theory, namely chain rule, for general membership problems, which encompasses both approximate and exact membership as extreme cases. Building upon the chain rule, we introduce a straightforward yet versatile algorithm framework, namely ChainedFilter, to combine different elementary filters without losing information. Our evaluation results demonstrate that ChainedFilter performs well in many applications: (1) it requires only 26% additional space over the theoretical lower bound for implicit static dictionary, (2) it requires only 0.22 additional bit per item over the theoretical lower bound for lossless data compression, (3) it reduces up to 31% external memory access than raw Cuckoo Hashing, (4) it reduces up to 36% P99 tail point query latency than Bloom Filter under the same space cost in RocksDB database, and (5) it reduces up to 99.1% filter space than original Learned Bloom Filter.

==> InputFiles/author_format.tex <==
\author{Tong Yang, Gaogang xie, Yanbiao Li, Qiaobin Fu, Alex X. Liu, Qi Li, Laurent Mathy}

\numberofauthors{6}
\author{
\alignauthor
Tong Yang,Gaogang Xie*\\
       %\affaddr{Institute of Computing Technology, Chinese Academy of Sciences (CAS), China.}\\
       \affaddr{ICT, CAS, China.}\\
       \email{yangtongemail@gmail.com, *xie@ict.ac.cn}
\alignauthor
YanBiao Li\\
       %\affaddr{College of Computer Science and Electronic Engineering, Hunan University, China}\\
       \affaddr{Hunan University, China}\\
       \email{lybmath\_cs@hnu.edu.cn}
\alignauthor
Qiaobin Fu\\
       \affaddr{ICT, CAS, China}\\
       \email{fuqiaobin@ict.ac.cn}
\and
\alignauthor Alex X. Liu\\
       \affaddr{Department of Computer Science and Engineering, Michigan State University}\\
       \email{alexliu@cse.msu.edu}
\alignauthor Qi Li\\
       \affaddr{ICT, CAS, China}\\
       \email{liqi19872006@gmail.com}
\alignauthor Laurent Mathy\\
       \affaddr{University of Liege, Belgium}\\
       \email{laurent.mathy@ulg.ac.be}
}


\author{\IEEEauthorblockN{Tong Yang\IEEEauthorrefmark{1},
Xiaoming Li\IEEEauthorrefmark{1},
Alex X. Liu\IEEEauthorrefmark{2},
Qiaobin Fu\IEEEauthorrefmark{3},
Gaogang Xie\IEEEauthorrefmark{4}}
\IEEEauthorblockA{\IEEEauthorrefmark{1}Computer Science Department, Peking University, Beijing, China}
\IEEEauthorblockA{\IEEEauthorrefmark{2}Department of Computer Science and Engineering, Michigan State University}
\IEEEauthorblockA{\IEEEauthorrefmark{3}Computer Science Department, Boston University, USA}
\IEEEauthorblockA{\IEEEauthorrefmark{4}ICT, CAS, China}
}

==> SIGMOD21/hwc/Figure/aae.tex <==
\begin{figure*}[!htbp]
	\centering
	%
	\hspace{-0.3in}
	\subfigure[CAIDA]{
		\begin{minipage}[t]{0.26\textwidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{SIGMOD21/hwc/Figure/CAIDAAAE2.pdf}
		\end{center}
		}
		\label{subfig:aae:syn}
		\end{minipage}
	}
	%
	\hspace{-0.3in}
	\subfigure[Webpage]{
		\begin{minipage}[t]{0.26\textwidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{SIGMOD21/hwc/Figure/WebpageAAE2.pdf}
		\end{center}
		}
		\label{subfig:fre:aae:ip}
		\end{minipage}
	}
	%
	\hspace{-0.3in}
	\subfigure[Network]{
		\begin{minipage}[t]{0.26\textwidth}{
		\begin{center}		
		\includegraphics[width=\textwidth, ]{SIGMOD21/hwc/Figure/NetworkAAE2.pdf}
		\end{center}
		}
		\label{subfig:fre:aae:web}
		\end{minipage}
	}
	%
	\hspace{-0.3in}
	\subfigure[Synthesis]{
		\begin{minipage}[t]{0.26\textwidth}{
		\begin{center}		
		\includegraphics[width=\textwidth]{SIGMOD21/hwc/Figure/synthe_AAE2.pdf}
		\end{center}
		}
		\label{subfig:fre:aae:net}
		\end{minipage}
	}
	%
    \caption{AAE of finding top-$K$ frequent items.}
	\label{fig:aae}
\end{figure*}

==> SIGMOD21/hwc/Figure/are.tex <==
\begin{figure*}[!htbp]
	\centering
	%
	\hspace{-0.3in}
	\subfigure[CAIDA]{
		\begin{minipage}[t]{0.26\textwidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{SIGMOD21/hwc/Figure/CAIDAARE2.pdf}
		\end{center}
		}
		\label{subfig:ARE:CAIDA}
		\end{minipage}
	}
	%
	\hspace{-0.3in}
	\subfigure[Webpage]{
		\begin{minipage}[t]{0.26\textwidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{SIGMOD21/hwc/Figure/WebpageARE2.pdf}
		\end{center}
		}
		\label{subfig:fre:ARE:webpage}
		\end{minipage}
	}
	%
	\hspace{-0.3in}
	\subfigure[Network]{
		\begin{minipage}[t]{0.26\textwidth}{
		\begin{center}		
		\includegraphics[width=\textwidth, ]{SIGMOD21/hwc/Figure/NetworkARE2.pdf}
		\end{center}
		}
		\label{subfig:fre:ARE:network}
		\end{minipage}
	}
	%
	\hspace{-0.3in}
	\subfigure[Synthesis]{
		\begin{minipage}[t]{0.26\textwidth}{
		\begin{center}		
		\includegraphics[width=\textwidth, ]{SIGMOD21/hwc/Figure/synthe_ARE2.pdf}
		\end{center}
		}
		\label{subfig:fre:ARE:synthe}
		\end{minipage}
	}
	%
    \caption{ARE of finding top-$K$ frequent items.}
	\label{fig:ARE}
\end{figure*}

==> SIGMOD21/hwc/Figure/bound.tex <==
\begin{figure}[!htbp]
	\centering
	%
	\subfigure[$\mathcal{P}$: SpaceSaving]{
		\begin{minipage}[t]{0.47\linewidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{SIGMOD21/hwc/Figure/bound2.pdf}
		\end{center}
		}
		\label{subfig:boundss}
		\end{minipage}
	}
	%
	\hspace{-0.1in}
	\centering
	\subfigure[$\mathcal{P}$: Randomized Admission Policy]{
		\begin{minipage}[t]{0.47\linewidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{SIGMOD21/hwc/Figure/bound3.pdf}
		\end{center}
		}
		\label{subfig:boundra}
		\end{minipage}
	}
	\caption{Sample variances and their theoretical upper bounds.}
	\label{fig:bound}
	
\end{figure}

==> SIGMOD21/hwc/Figure/compare.tex <==
\begin{figure}[!htbp]
    \centering
    \includegraphics[width=0.6\linewidth]{SIGMOD21/hwc/Figure/compare.pdf}
    \caption{ARE Comparisons between the Basic Version and the Optimized Version of UTF.
    }
    \label{fig:Compare}
\end{figure}

==> SIGMOD21/hwc/Figure/global_topk.tex <==

\begin{figure*}[!htbp]
	\centering
	%
	\hspace{-0.1in}
	\subfigure[\revise{Overall Performance: F1 Score}]{
		\begin{minipage}[t]{0.245\textwidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{SIGMOD21/hwc/Figure/global_skewed_f1_weighted.pdf}
		\end{center}
		}
		\label{subfig:global_topk:f1}
		\end{minipage}
	}
	%
	\hspace{-0.1in}
	\subfigure[\revise{\Fairness{}: Relative Bias}]{
		\begin{minipage}[t]{0.245\textwidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{SIGMOD21/hwc/Figure/global_skewed_rb_weighted.pdf}
		\end{center}
		}
		\label{subfig:global_topk:bias}
		\end{minipage}
	}
	%
	\hspace{-0.1in}
	\subfigure[\revise{Recall on Aggregation of light machines}]{
		\begin{minipage}[t]{0.245\textwidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{SIGMOD21/hwc/Figure/global_skewed_roal_weighted.pdf}
		\end{center}
		}
		\label{subfig:global_topk:small}
		\end{minipage}
	}
	%
	\subfigure[\revise{Recall on Aggregation of heavy machines}]{
		\begin{minipage}[t]{0.245\textwidth}{
		\begin{center}		
		\includegraphics[width=\textwidth, ]{SIGMOD21/hwc/Figure/global_skewed_roa_weighted.pdf}
		\end{center}
		}
		\label{subfig:global_topk:large}
		\end{minipage}
	}
	%
    \caption{\revise{Performance and fairness of weighted algorithms for finding global top-$K$ items.}}
	\label{fig:global_topk}
\end{figure*}

==> SIGMOD21/hwc/Figure/global_topk_demo.tex <==
\begin{figure}[!htbp]
	\centering
	%
	\centering
	\subfigure[Recall of the global top-1 flow]{
		\begin{minipage}[t]{0.45\linewidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{SIGMOD21/hwc/Figure/top-1-ranking.pdf}
		\end{center}
		}
		\label{subfig:global-top1-rc-demo}
		\end{minipage}
	}
	%
	\subfigure[Top-1 flow's average estimated global ranking]{
		\begin{minipage}[t]{0.45\linewidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{SIGMOD21/hwc/Figure/top-1-ranking.pdf}
		\end{center}
		}
		\label{subfig:global-top1-ranking-demo}
		\end{minipage}
	}
	\caption{We demonstrate why conditional unbiasedness is important in the global top-$K$ task. We show that when memory is extremely tight, the unfairness comparison of conditionally biased algorithms during the aggregation of top-$K$ flows would lead to severe performance degradation so that even the real top-1 flow may not be reported as global top-$K$ item.}
	\label{fig:global-topk-demo}
	
\end{figure}

==> SIGMOD21/hwc/Figure/global_topk_overall.tex <==
\begin{figure*}[!t]
	\centering
	%
	\hspace{-0.2in}
	\subfigure[CAIDA]{
		\begin{minipage}[t]{0.25\textwidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{SIGMOD21/hwc/Figure/global_overall_caida_ARE.pdf}
		\end{center}
		}
		\label{subfig:global_overall_caida_ARE}
		\end{minipage}
	}
	%
	\hspace{-0.2in}
	\subfigure[Webpage]{
		\begin{minipage}[t]{0.26\textwidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{SIGMOD21/hwc/Figure/global_overall_web_ARE.pdf}
		\end{center}
		}
		\label{subfig:global_overall_web_ARE}
		\end{minipage}
	}
	\hspace{-0.2in}
	%
	\subfigure[Net]{
		\begin{minipage}[t]{0.26\textwidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{SIGMOD21/hwc/Figure/global_overall_net_ARE.pdf}
		\end{center}
		}
		\label{subfig:global_overall_net_ARE}
		\end{minipage}
	}
	%
	\hspace{-0.2in}
	\subfigure[Synthesis]{
		\begin{minipage}[t]{0.25\textwidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{SIGMOD21/hwc/Figure/global_overall_syn_ARE.pdf}
		\end{center}
		}
		\label{subfig:global_overall_syn_ARE}
		\end{minipage}
	}
	%
    \caption{ARE on finding global top-$K$ items.}
	\label{fig:global_overall_ARE}
\end{figure*}

\begin{figure*}[!t]
	\centering
	%
	\hspace{-0.2in}
	\subfigure[CAIDA]{
		\begin{minipage}[t]{0.25\textwidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{SIGMOD21/hwc/Figure/global_overall_caida_F1.pdf}
		\end{center}
		}
		\label{subfig:global_overall_caida_F1}
		\end{minipage}
	}
	%
	\hspace{-0.2in}
	\subfigure[Webpage]{
		\begin{minipage}[t]{0.26\textwidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{SIGMOD21/hwc/Figure/global_overall_web_F1.pdf}
		\end{center}
		}
		\label{subfig:global_overall_webpage_F1}
		\end{minipage}
	}
	%
	\hspace{-0.2in}
	\subfigure[Net]{
		\begin{minipage}[t]{0.26\textwidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{SIGMOD21/hwc/Figure/global_overall_net_F1.pdf}
		\end{center}
		}
		\label{subfig:global_overall_net_F1}
		\end{minipage}
	}
	%
	\hspace{-0.2in}
	\subfigure[Synthesis]{
		\begin{minipage}[t]{0.25\textwidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{SIGMOD21/hwc/Figure/global_overall_syn_F1.pdf}
		\end{center}
		}
		\label{subfig:global_overall_syn_F1}
		\end{minipage}
	}
	%
    \caption{F1 Score on finding global top-$K$ items.}
	\label{fig:global_overall_F1}
\end{figure*}


\begin{figure*}[!t]
	\centering
	%
	\hspace{-0.2in}
	\subfigure[CAIDA]{
		\begin{minipage}[t]{0.25\textwidth}{
		\begin{center}		
		\includegraphics[width=\textwidth, ]{SIGMOD21/hwc/Figure/local_topk_th.pdf}
		\end{center}
		}
		\label{subfig:global_overall_caida_th}
		\end{minipage}
	}
	%
	\hspace{-0.2in}
	\subfigure[Webpage]{
		\begin{minipage}[t]{0.26\textwidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{SIGMOD21/hwc/Figure/WebpageTh.pdf}
		\end{center}
		}
		\label{subfig:global_overall_webpage_th}
		\end{minipage}
	}
	%
	\hspace{-0.2in}
	\subfigure[Net]{
		\begin{minipage}[t]{0.26\textwidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{SIGMOD21/hwc/Figure/NetworkTh.pdf}
		\end{center}
		}
		\label{subfig:global_overall_net_th}
		\end{minipage}
	}
	%
	\hspace{-0.2in}
	\subfigure[Synthesis]{
		\begin{minipage}[t]{0.25\textwidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{SIGMOD21/hwc/Figure/synthe_Th.pdf}
		\end{center}
		}
		\label{subfig:global_overall_syn_th}
		\end{minipage}
	}
	%
    \caption{Throughput on finding global top-$K$ items.}
	\label{fig:global_overall_Th}
\end{figure*}



==> SIGMOD21/hwc/Figure/intro_demo.tex <==
\begin{figure}[!htbp]
    \vspace{-0.2in}
	\centering
	\subfigure[Internal unfairness]{
		\begin{minipage}[t]{0.45\linewidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{SIGMOD21/hwc/Figure/internal_unfair_demo.pdf}
		\end{center}
		}
		\label{subfig:intro-internal-unfair}
		\end{minipage}
	}
	%
	\hspace{-0.2in}
	\subfigure[Recall of the Global Top-1 Item]{
		\begin{minipage}[t]{0.45\linewidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{SIGMOD21/hwc/Figure/top-1-recall-2.pdf}
		\end{center}
		}
		\label{subfig:intro-recall-top-1}
		\end{minipage}
	}
	\caption{We demonstrate internal unfairness of USS, and show how external unfairness would severely harm accuracy for finding global top-$K$ items.}
	% 不是conditional unbiased怎样表述?
	\label{fig:intro-demo}
	
\end{figure}

==> SIGMOD21/hwc/Figure/local_topk.tex <==

\begin{figure*}[t!]
	
	\hspace{-0.2in}
	\subfigure[CAIDA: ARE]{
		\begin{minipage}[t]{0.25\textwidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{SIGMOD21/hwc/Figure/local_topk_ARE.pdf}
		\end{center}
		}
		\label{subfig:local_topk:caida-ARE}
		\end{minipage}
	}
	%
	\hspace{-0.3in}
	\subfigure[Synthetic: ARE]{
		\begin{minipage}[t]{0.25\textwidth}{
		\begin{center}		
		\includegraphics[width=\textwidth, ]{SIGMOD21/hwc/Figure/synthe_ARE.pdf}
		\end{center}
		}
		\label{subfig:local_topk:synthetic-ARE}
		\end{minipage}
	}
	%
	\hspace{-0.1in}
	\subfigure[CAIDA: F1 Score]{
		\begin{minipage}[t]{0.25\textwidth}{
		\begin{center}		
		\includegraphics[width=\textwidth, ]{SIGMOD21/hwc/Figure/local_topk_F1.pdf}
		\end{center}
		}
		\label{subfig:local_topk:caida-F1}
		\end{minipage}
	}
	%
	\hspace{-0.25in}
	\subfigure[Synthetic: F1 Score]{
		\begin{minipage}[t]{0.25\textwidth}{
		\begin{center}		
		\includegraphics[width=\textwidth, ]{SIGMOD21/hwc/Figure/synthe_F1.pdf}
		\end{center}
		}
		\label{subfig:local_topk_synthetic-F1}
		\end{minipage}
	}
    \caption{Performance of finding local top-$K$ items.}
	\label{fig:local_topk}
\end{figure*}

\begin{figure*}[!t]
	\centering
	%
	\hspace{-0.2in}
	\subfigure[Zero Error Rate]{
		\begin{minipage}[t]{0.25\textwidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{SIGMOD21/hwc/Figure/zero_error_rate.pdf}
		\end{center}
		}
		\label{subfig:local_topk:zero_error_rate}
		\end{minipage}
	}
	%
	\hspace{-0.2in}
	\subfigure[ARE of three Double-Anonymous Sketch versions]{
		\begin{minipage}[t]{0.25\textwidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{SIGMOD21/hwc/Figure/compare_are.pdf}
		\end{center}
		}
		\label{subfig:local_topk:three-version-are}
		\end{minipage}
	}
	%
	\hspace{-0.2in}
	\subfigure[Overestimation]{
		\begin{minipage}[t]{0.25\textwidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{SIGMOD21/hwc/Figure/overestimate.pdf}
		\end{center}
		}
		\label{subfig:overestimate}
		\end{minipage}
	}
	%
	\hspace{-0.2in}
	\subfigure[Underestimation]{
		\begin{minipage}[t]{0.25\textwidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{SIGMOD21/hwc/Figure/underestimate.pdf}
		\end{center}
		}
		\label{subfig:underestimate}
		\end{minipage}
	}
    \caption{Performance on zero error rate, comparisons between the three versions, and performance on providing overestimation and underestimation of items' frequency for finding local top-$K$ items.}
	\label{fig:local_topk-others}
\end{figure*}

==> SIGMOD21/hwc/Figure/more_ds.tex <==
\begin{figure*}[!htbp]
	\centering
	%
	\hspace{-0.3in}
	\subfigure[Webpage]{
		\begin{minipage}[t]{0.26\textwidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{SIGMOD21/hwc/Figure/global_overall_web_ARE.pdf}
		\end{center}
		}
		\label{subfig:global_overall_web_ARE}
		\end{minipage}
	}
	%
	\hspace{-0.3in}
	\subfigure[Net]{
		\begin{minipage}[t]{0.26\textwidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{SIGMOD21/hwc/Figure/global_overall_net_ARE.pdf}
		\end{center}
		}
		\label{subfig:global_overall_net_ARE}
		\end{minipage}
	}
	%
	\hspace{-0.3in}
	\subfigure[Webpage]{
		\begin{minipage}[t]{0.26\textwidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{SIGMOD21/hwc/Figure/global_overall_caida_F1.pdf}
		\end{center}
		}
		\label{subfig:global_overall_webpage_F1}
		\end{minipage}
	}
	%
	\hspace{-0.3in}
	\subfigure[Net]{
		\begin{minipage}[t]{0.26\textwidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{SIGMOD21/hwc/Figure/global_overall_syn_F1.pdf}
		\end{center}
		}
		\label{subfig:global_overall_net_F1}
		\end{minipage}
	}
	%
    \caption{More experimental results on different datasets for finding global top-$K$ items.}
	\label{fig:more_ds}
\end{figure*}

==> SIGMOD21/hwc/Figure/overunderestimateare.tex <==
\begin{figure}[!htbp]
	\centering
	%
	\hspace{-0.1in}
	\subfigure[Overestimation]{
		\begin{minipage}[t]{0.25\textwidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{SIGMOD21/hwc/Figure/overestimate.pdf}
		\end{center}
		}
		\label{subfig:overestimate}
		\end{minipage}
	}
	%
	\hspace{-0.3in}
	\subfigure[Underestimation]{
		\begin{minipage}[t]{0.25\textwidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{SIGMOD21/hwc/Figure/underestimate.pdf}
		\end{center}
		}
		\label{subfig:underestimate}
		\end{minipage}
	}
    \caption{ARE of overestimation and underestimation on finding local top-$K$ items.}
	\label{fig:overunderestimation}
\end{figure}

==> SIGMOD21/hwc/Figure/recall.tex <==
\begin{figure*}[!htbp]
	\centering
	%
	\hspace{-0.3in}
	\subfigure[CAIDA]{
		\begin{minipage}[t]{0.26\textwidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{SIGMOD21/hwc/Figure/CAIDARc2.pdf}
		\end{center}
		}
		\label{subfig:rec:CAIDA}
		\end{minipage}
	}
	%
	\hspace{-0.3in}
	\subfigure[Webpage]{
		\begin{minipage}[t]{0.26\textwidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{SIGMOD21/hwc/Figure/WebpageRc2.pdf}
		\end{center}
		}
		\label{subfig:fre:rec:Web}
		\end{minipage}
	}
	%
	\hspace{-0.3in}
	\subfigure[Network]{
		\begin{minipage}[t]{0.26\textwidth}{
		\begin{center}		
		\includegraphics[width=\textwidth, ]{SIGMOD21/hwc/Figure/NetworkRc2.pdf}
		\end{center}
		}
		\label{subfig:fre:rec:Net}
		\end{minipage}
	}
	%
	\hspace{-0.3in}
	\subfigure[Synthesis]{
		\begin{minipage}[t]{0.26\textwidth}{
		\begin{center}		
		\includegraphics[width=\textwidth, ]{SIGMOD21/hwc/Figure/synthe_Rc2.pdf}
		\end{center}
		}
		\label{subfig:fre:rec:syn}
		\end{minipage}
	}
	%
    \caption{F1 scores of finding top-$K$ frequent items.}
	\label{fig:recall}
\end{figure*}

==> SIGMOD21/hwc/Figure/skewness.tex <==
\begin{figure}[!htbp]
	\centering
	%
	\centering
	\subfigure[F1 Score]{
		\begin{minipage}[t]{0.45\linewidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{SIGMOD21/hwc/Figure/skewnessRc2.pdf}
		\end{center}
		}
		\label{subfig:skewnessRc}
		\end{minipage}
	}
	%
	\subfigure[ARE]{
		\begin{minipage}[t]{0.45\linewidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{SIGMOD21/hwc/Figure/skewness_ARE2.pdf}
		\end{center}
		}
		\label{subfig:skewnessare}
		\end{minipage}
	}
	\caption{Evaluations on dataset Skewness.}
	\label{fig:skewness}
	
\end{figure}

==> SIGMOD21/hwc/Figure/throughput.tex <==
\begin{figure*}[!htbp]
	\centering
	%
	\hspace{-0.3in}
	\subfigure[CAIDA]{
		\begin{minipage}[t]{0.26\textwidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{SIGMOD21/hwc/Figure/CAIDATh2.pdf}
		\end{center}
		}
		\label{subfig:Th:CAIDA}
		\end{minipage}
	}
	%
	\hspace{-0.3in}
	\subfigure[Webpage]{
		\begin{minipage}[t]{0.26\textwidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{SIGMOD21/hwc/Figure/WebpageTh2.pdf}
		\end{center}
		}
		\label{subfig:fre:Th:Web}
		\end{minipage}
	}
	%
	\hspace{-0.3in}
	\subfigure[Network]{
		\begin{minipage}[t]{0.26\textwidth}{
		\begin{center}		
		\includegraphics[width=\textwidth, ]{SIGMOD21/hwc/Figure/NetworkTh2.pdf}
		\end{center}
		}
		\label{subfig:fre:Th:Net}
		\end{minipage}
	}
	%
	\hspace{-0.3in}
	\subfigure[Synthesis]{
		\begin{minipage}[t]{0.26\textwidth}{
		\begin{center}		
		\includegraphics[width=\textwidth, ]{SIGMOD21/hwc/Figure/synthe_Th2.pdf}
		\end{center}
		}
		\label{subfig:fre:Th:syn}
		\end{minipage}
	}
	%
    \caption{Throughput of finding top-$K$ frequent items.}
	\label{fig:Th}
\end{figure*}

==> SIGMOD21/hwc/Figure/unbiasedness.tex <==
\begin{figure}[!htbp]
	\centering
	%
	\subfigure[Unbiased estimations of UTF]{
		\begin{minipage}[t]{0.5\linewidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{SIGMOD21/hwc/Figure/unbiasedness.pdf}
		\end{center}
		}
		\label{subfig:unbiasedness-UTF}
		\end{minipage}
	}
	%
	\hspace{-0.3in}
	\subfigure[Estimations of USS]{
		\begin{minipage}[t]{0.5\linewidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{SIGMOD21/hwc/Figure/uss_unbiase_compare.pdf}
		\end{center}
		}
		\label{subfig:biasedness-USS}
		\end{minipage}
	}
	\caption{Distributions of estimated frequencies of UTF and USS. It can be concluded that UTF achieves unbiased on the \textit{reported} top-$K$ items, while USS is biased on the \textit{reported} top-$K$ items.}
	\label{fig:demonstrations}
	
\end{figure}

==> SIGMOD21/hwc/Figure/varying_k.tex <==
\begin{figure}[!htbp]
	\centering
	%
	\subfigure[ARE]{
		\begin{minipage}[t]{0.45\linewidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{SIGMOD21/hwc/Figure/varying_k_ARE.pdf}
		\end{center}
		}
		\label{subfig:varying-k-ARE}
		\end{minipage}
	}
	%
	\centering
	\subfigure[F1 Score]{
		\begin{minipage}[t]{0.45\linewidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{SIGMOD21/hwc/Figure/varying_k_rc.pdf}
		\end{center}
		}
		\label{subfig:varying-k-rc}
		\end{minipage}
	}
	\caption{Evaluations on different $K$.}
	\label{fig:varying-k}
	
\end{figure}

==> SIGMOD21/hwc/Figure/varying_params.tex <==
\begin{figure*}[!htbp]
	\centering
	%
	\hspace{-0.2in}
	\subfigure[Varying $\lambda$: ARE]{
		\begin{minipage}[t]{0.26\textwidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{SIGMOD21/hwc/Figure/varying_d_are.pdf}
		\end{center}
		}
		\label{subfig:varying-lambda-are}
		\end{minipage}
	}
	%
	\hspace{-0.2in}
	\subfigure[Varying $\lambda$: Throughput]{
		\begin{minipage}[t]{0.26\textwidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{SIGMOD21/hwc/Figure/varying_d_th.pdf}
		\end{center}
		}
		\label{subfig:varying-lambda-th}
		\end{minipage}
	}
	%
	\hspace{-0.2in}
	\subfigure[Varying $M_{top-K}/M$: ARE]{
		\begin{minipage}[t]{0.26\textwidth}{
		\begin{center}		
		\includegraphics[width=\textwidth, ]{SIGMOD21/hwc/Figure/varying_ratio_ARE.pdf}
		\end{center}
		}
		\label{subfig:varying-ratio_ARE}
		\end{minipage}
	}
	%
	\hspace{-0.2in}
	\subfigure[Varying $\frac{M_{top-K}}{M}$: F1 Score]{
		\begin{minipage}[t]{0.26\textwidth}{
		\begin{center}		
		\includegraphics[width=\textwidth, ]{SIGMOD21/hwc/Figure/varying_ratio_rc.pdf}
		\end{center}
		}
		\label{subfig:varying-ratio_rc}
		\end{minipage}
	}
	%
    \caption{Experiments on different parameter settings ($\lambda$ and $\frac{M_{top-K}}{M}$) of Double-Anonymous Sketch.}
	\label{fig:varying-params}
\end{figure*}


==> SIGMOD21/hwc/exp_unbiasedness.tex <==
\subsection{Demonstrations of Unbiasedness, and Over Estimation and Under Estimation of UTF}
\label{sec:experiment-unbiasedness}

We have conducted experiments to demonstrate the unbiasedness of our algorithm, and to demonstrate that UTF can provide overestimation and underestimation values (figure \ref{fig:demonstrations} \footnote{Some distinct items with extremely large $f$ are omitted for better demonstration}). 

\ppp{Unbiasedness}: In figure \ref{subfig:unbiasedness}, we perform experiment of UTF+RA in our default settings \textbf{one time}, and we plot data points:$(f_i, \hat{f}_i-f_i)$ of top 200 correctly reported top-k items in this figure, where $f_i$ is the real frequency and $\hat{f}_i$ is the unbiased estimation. We find that the data points scatter almost equally below and above the $x$-axis, which verifies the unbiasedness of UTF. In figure \ref{subfig:average-error}, we demonstrate the average total error value in different experiments (with the same settings), where average total error $=\frac{1}{\mathbf{\Psi}}\sum_{e_i \in \mathbf{\Psi}}(f_i - \hat{f}_i)$. The fact that data points scatter around line $y=0$ also supports this conclusion.

\ppp{overestimation and underestimation}: In section \ref{sec:generity}, we show that UTF can not only provide the unbiased estimations of the items' frequency, but also provide over estimations and under estimations. Figure \ref{subfig:overunderestimation} demonstrates the distributions of under estimations and over estimations of top-k frequent items. 



==> SIGMOD21/hwc/experiment.tex <==
%% 可能一些不重要的实验图需要删减: 例如变化$k$的实验图.




%\input{SIGMOD21/hwc/Figure/aae}
%\input{SIGMOD21/hwc/Figure/are}



%%







%% Experimental results
\presec
\section{Experimental Results}

\label{sec:experiments}
%% In this section, we provide our experimental results. %% In section xxx.



% \input{SIGMOD21/hwc/exp_unbiasedness}

%\input{SIGMOD21/hwc/Figure/recall}
%\input{SIGMOD21/hwc/Figure/throughput}

\input{SIGMOD21/hwc/Figure/local_topk}

\input{SIGMOD21/hwc/setup}


\input{SIGMOD21/hwc/Figure/global_topk_overall}

\input{SIGMOD21/hwc/local_topk}

% \input{SIGMOD21/hwc/Figure/overunderestimateare}


\input{SIGMOD21/hwc/Figure/global_topk}



\input{SIGMOD21/hwc/global_topk}



\input{SIGMOD21/hwc/param_settings}

% \input{SIGMOD21/hwc/Figure/varying_params}






% \input{SIGMOD21/hwc/Figure/skewness}


% \input{SIGMOD21/hwc/Figure/varying_k}


%\input{SIGMOD21/hwc/Figure/compare}


%\input{SIGMOD21/hwc/over_under_est}



% \input{SIGMOD21/hwc/param_settings}
%%
% \input{SIGMOD21/hwc/verify_bound}



==> SIGMOD21/hwc/global_topk.tex <==
\presub
\subsection{Experiments on Global Top-$K$ with Same Sizes across Different Data Streams}
\postsub
\label{sec:global_topk_balanced}


\input{tex/fig/fig6}

\remove{
In a distributed scenario, there are $N$ data streams $\mathcal{S}_1, \cdots, \mathcal{S}_N$.  Data stream $\mathcal{S}_i$ contains $n_i$ items, and different data streams contain disjoint items. Each data stream is measured by a sketch on one machine. Memory sizes of all the sketches on different data streams are set the same since we cannot know the number of items $n_i$ of each data stream in advance. We denote $M$ as the total memory sizes of all the sketches, and $S = \bigcup_{i=1}^N \mathcal{S}_i$. On insertion, each incoming item is inserted into its corresponding sketch. On querying, each sketch $i$ returns its local top-$K$ items along with their estimated frequencies: $\mathcal{T}_i = \{(e_j, \hat{f_j})|j=1 \cdots K\}$. The global top-$K$ selector unions all the local top-$K$ items and selects the top-$K$ largest items as global top-$K$ items. 
%
In different application scenarios, the skewness of the size distribution across different data streams could be small or large.  We set $n_1 = r*|\mathcal{S}|$, and $n_i = \frac{1-r}{N-1}|\mathcal{S}|, i \ge 2$, where $r \ge \frac{1}{N}$ represents the skewness of the size distribution across different data streams. We denote $\mathcal{S}_1$ as a heavy stream, and other data streams as light streams. In this subsection, we focus on the case when the sizes of different data streams are the same, \ie, $r=\frac{1}{N}$.
}

\update{
\ppp{Application Description}:
%
In a distributed scenario, there are $N$ data streams $\mathcal{S}_1, \cdots, \mathcal{S}_N$. 
%
Data stream $\mathcal{S}_i$ contains $m_i$ items.
%
Each data stream is measured by a sketch on one machine. 
%
Memory sizes of all the sketches on different data streams are set the same.
%
We denote $\mathcal{S} = \bigcup_{i=1}^N \mathcal{S}_i$.
%
In different scenarios, the skewness of the size distribution across different data streams could be small or large. 
%
We set $m_1 = r*|\mathcal{S}|$, and $m_i = \frac{1-r}{N-1}|\mathcal{S}|, i \ge 2$, where $r \ge \frac{1}{N}$ represents the skewness of the size distribution across different data streams. 
%
We denote $\mathcal{S}_1$ as a heavy stream, and other data streams as light streams. 
%
In this subsection, we focus on the case when the sizes of different data streams are the same, \ie, $r=\frac{1}{N}$.
}

\ppp{Experimental settings}: We use all the four datasets mentioned in \ref{sec:experimental-setup-datasets} for our experiments. There are in total $N=10$ data streams, and we select $K=1000$ global top-$K$ items. We allocate the same amount of memory for each sketch on different machines, and the total memory size for the $N=10$ sketches in total ranges from $100$KB to $500$KB. 


\ppp{ARE (Figure \ref{subfig:global_overall_caida_ARE} - \ref{subfig:global_overall_syn_ARE})}: We find that our approach could achieve much lower ARE than prior art. On CAIDA dataset, when $M=100$KB, ARE of our approach is 3 orders of magnitude times lower than Frequent, USS, SS, and $70$ times lower than Waving. We observe similar results on the other three datasets.

\ppp{F1 Score (Figure \ref{subfig:global_overall_caida_F1} - \ref{subfig:global_overall_syn_F1})}: Results show that in this scenario, our approach could achieve a high F1 Score on both datasets even when $M$ is small. When $M=100$KB, the F1 Score of our approach is greater than $90\%$ on both datasets, while the F1 Score of Frequent, USS, and SS is lower than $60\%$ on the Webpage dataset and lower than $40\%$ on the rest of the datasets. We also find that our approach achieves a slightly better F1 Score than Waving .

\ppp{Throughput (Table \ref{table:throughput})}: Our approach achieves higher or comparable throughput compared with prior art. Specifically, the throughput of our approach is on average $3.19$, $2.89$ and $3.15$ times higher than Frequent, USS, and SS respectively over the four datasets, and is comparable with Waving. 




\begin{table}[!ht]
    \setlength{\abovecaptionskip}{-0.0cm}
    \setlength{\belowcaptionskip}{-0.0cm}
\centering
    \begin{tabular}{|c|c|c|c|c|}
        \hline
        & CAIDA & Webpage & Net & Synthesis \\ \hline
        Frequent (300KB) & 5.3 & 6.2 & 4.5 & 5.1 \\ \hline
        USS (300KB) & 5.4 & 6.9 & 5.3 & 5.7 \\ \hline
        SS (300KB) & 5.9 & 6.4 & 4.8 & 4.7 \\ \hline
        Waving (300KB) & 14.8 & 21.2 & 13.4 & 16.8 \\ \hline
        Ours + RA (300KB) & 14.9 & 25.5 & 12.7 & 15.6 \\ \hline
    \end{tabular}
    \caption{\revise{Throughput (Mops) of finding top-$K$ frequent items.}}
    \label{table:throughput}
\end{table}

\ppp{Analysis}:
1) Our approach is accurate in frequency estimation on global top-$K$ items even with extremely small memory. Prior works, like Frequent, USS, and SS tend to provide highly underestimated or overestimated frequency estimation, so their frequency estimation tends to be significantly inaccurate. Waving sketch is also not as accurate as our approach because when memory is tight, Waving counters tend to be highly inaccurate.
%
2) F1 Score of our approach is mainly determined by the top-$K$ replacement strategy, and when applying Randomized Admission Policy (RA) replacement strategy to our approach, the Double-Anonymous sketch could achieve a high F1 Score on both the local top-$K$ task and the global top-$K$ task. F1 Score of Frequent, USS, and SS is significantly lower than our approach since all of them use the Stream Summary \cite{spacesaving} data structure, which consumes more memory to store one item than our approach, and those replacement strategies are not as accurate as the RA replacement strategy. 
%
3) Both our approach and Waving sketch use bucket-array data structure, which is cache-friendly and requires fewer memory access, resulting in higher insertion throughput. For Frequent, USS, and SS, frequent pointer operations would lead to cache misses, making the insertion much slower. 



\subsection{Experiments on \Fairness{} with Highly Skewed Data Streams' Sizes\\}
\label{sec:global_topk_imbalanced}


\bbb{5.4.1 Experimental Setup}
\\

In this subsection, we focus on the case when the size distribution is highly skewed. 
%
We show why \fairness{} is important in finding global top-$K$ items in this scenario.
%
\update{
We apply four replacement policies to the Double-Anonymous sketch and compare our results with four biased algorithms: Frequent, SS, HG, and RA, and two unbiased algorithms: USS, and Waving.
}
%
\revise{
\textbf{F1 Score} is used to demonstrate the overall performance of those algorithms. 
%
\textbf{Relative bias} is used to directly demonstrate the \fairness{} of our approach and the \unfairness{} of prior art.
}
%
Considering the global top-$K$ aggregation: 
%
before that, sketch $i$ proposes several local top-$K$ candidates, and some of them are real global top-$K$ items.
%
Among those real global top-$K$ items proposed by sketch $i$, only a proportion of them survive and are selected as global top-$K$ items. 
%
\textbf{Recall on aggregation}, which refers to the proportion mentioned above, is used to demonstrate the \fairness{} of the global top-$K$ selector on aggregation. 
%
Specifically, we use this metric to answer our questions:
%
\textit{does the global top-$K$ selector favors items from heavy machines or from light machines, or is the global \fair{} so that it selects global top-$K$ items solely based only on their real frequency, regardless of which local sketch it comes from.}

\begin{table}[!ht]
    \setlength{\abovecaptionskip}{-0.0cm}
    \setlength{\belowcaptionskip}{-0.0cm}
\centering
    \begin{tabular}{|c|c|c|c|c|c|c|}
        \hline
        Frequent & SS & HG & RA & USS & Waving & Ours \\ \hline
        $40$KB & $40$KB & $15$KB & $15$KB & $40$KB & $15$KB & $15$KB \\ \hline
    \end{tabular}
    \caption{Memory size configurations in Section \ref{sec:global_topk_imbalanced}}
    \label{table:memory_size}
\end{table}


\ppp{Experimental Settings}: We set $N=100$, $K=1000$, and vary the skewness $r$ from $0.01$ to $0.5$. 
%
In order to better demonstrate how \fairness{} affects the performance and eliminate the effects of selecting local top-$K$ items itself on the performance of finding global top-$K$ items, we adjust the memory sizes for different algorithms so that they could store exactly the same number of local top-$K$ candidates.
%
The configurations on memory size are shown in Table~ \ref{table:memory_size}. We use the synthetic dataset with skewness=$0.9$, which is relatively low in skewness, to better demonstrate the concept of "\fairness{}" and illustrate our results. 
\\



\input{SIGMOD21/hwc/Figure/global_topk}

\bbb{5.4.2 Overall Performance \& \Fairness{}}
\\

\ppp{F1 Score (Figure \ref{subfig:global_topk_1:f1} and \ref{subfig:global_topk_2:f1})}: 
%
\zyk{
Results show that when skewness increases, our F1 Score degradation is much slower than all the prior art.
%
Specifically, when skewness $r = 0.5$, Ours + Frequent achieves F1 Score $\ge 73\%$, while Frequent itself only achieves F1 Score $\le 48\%$; 
%
Ours + SS achieves F1 Score $\ge 72\%$, while SS itself only achieves F1 Score $\le 31\%$. 
%
Ours + RA achieves F1 Score $\ge 98\%$, while RA itself only achieves F1 Score $\le 83\%$. 
%
Ours + HG achieves F1 Score $\ge 95\%$, while HG itself only achieves F1 Score $\le 76\%$. 
%
F1 Score of Waving Sketch and USS is $62\%$, $30\%$ respectively, which is also significantly lower than that of our approach.
}

\ppp{Relative Bias on Top-$K$ items (Figure \ref{subfig:global_topk_1:bias} and \ref{subfig:global_topk_2:bias})}: 
%
\zyk{
\hypertarget{link:exp_rep_1}{Results} show that SS, USS and Waving tend to provide overestimated frequency. 
%
For these algorithms, items in heavy machines tend to be overestimated much more than light machines, so the global top-$K$ selector tends to favor items in heavy machines.
%
Similarly, Frequent, RA, and HG tend to provide underestimated frequency, and items in heavy machines tend to be underestimated much more, so the global top-$K$ selector tends to favor items in light machines.
%
More detailed recall rates on aggregation are shown in Section 5.4.3.
}

\ppp{Analysis}:
1) One of the desired properties that \fairness{} brings is that the F1 Score of \fair{} algorithms, like our Double-Anonymous sketch, tends to be higher than \unfair{} algorithms. 
%
For example, for SS and USS, local top-$K$ candidates in heavy machines tend to be highly overestimated, so even if an item in heavy machines is low in real frequency, its estimated frequency is still high enough to be falsely selected as a global top-$K$ item.
%
With items in heavy machines falsely selected as global top-$K$ items and items in light machines ignored, the F1 Scores of SS and USS become unacceptably low when skewness is large.
%
\zyk{
\hypertarget{link:disc_rep_1}{2)} The degree of \unfairness{} of algorithms is often negatively related to their F1 scores.
%
Specifically, the \unfairness{} of SS, USS, and Frequent is very significant, so their F1 scores are lower than other algorithms.
%
Although Waving, RA, and HG are also \unfair{}, their \unfairness{} is relatively slight, so they have higher F1 scores.
%
For \fair{} algorithms, the accuracy of the replacement policy they use determines their performance, so Ours+RA and Ours+HG have the highest F1 scores.
}
%
3) Our approach is generic: we can make \textit{any} top-$K$ algorithm \fair{} simply by applying the Double-Anonymous sketch to this top-$K$ algorithm. 
%
Meanwhile, the F1 Score is also much improved because our approach is \fair{} in global top-$K$ aggregation.
%
\zyk{
Specifically, for top-$K$ algorithms Frequent and SS with significant \unfairness{}, our DA sketch can improve their F1 scores by up to 25.5\% and 42.5\%; and for top-$K$ algorithms RA and HG with slight \unfairness{}, our DA sketch can still improve their F1 scores by 15.0\% and 19.8\%.
\\
}


\bbb{5.4.3 Recall on Aggregation}
\\

\ppp{Recall on Aggregation (Figure \ref{subfig:global_topk_1:small} - \ref{subfig:global_topk_1:large} and \ref{subfig:global_topk_2:small} - \ref{subfig:global_topk_2:large})}: 
%
\zyk{
For light machines, we find that Recall on Aggregation of overestimation algorithms, like SS, USS, and Waving, decreases fast as $r$ increases, while that of other algorithms keeps at a high level ($\ge 90\%$).
%
Conversely, for heavy machines, Recall on Aggregation of underestimation algorithms like Frequent, RA, and HG, decreases as $r$ increases, while other algorithms remain $\ge 90\%$.
}
%
It can be concluded that for overestimation algorithms, it is more difficult for items in light machines to survive the global aggregation and be selected as global top-$K$ items;
%
for underestimation algorithms, it is more difficult for items in heavy machines to be selected as global top-$K$ items.

\input{SIGMOD21/hwc/Figure/varying_params}

\revise{
\ppp{Analysis}:
\hypertarget{link:disc_rep_2}{\Fairness{}} is determined by the bias of frequency estimation on top-$K$ items. 
%
For overestimation sketches like SS, USS, and Waving, many local top-$K$ candidates from light machines that are supposed to become global top-$K$ items would actually be evicted during aggregation (Recall on Aggregation on light machines tends to be small). 
%
It can be concluded that the global top-$K$ selector favors items from heavy machines. 
%
Conversely, for underestimation sketches like Frequent, RA, and HG, global top-$K$ selector tends to favors items from light machines.
%
We argue that \unfair{} aggregation is unacceptable in many real-world applications since the global top-$K$ selector should not be partial to items from any machine.
\\
}

\remove{
\ppp{Analysis}:
1) \Fairness{} is determined by the bias of frequency estimation on top-$K$ items. For overestimation sketches like SS, USS, and Waving, many local top-$K$ candidates from light machines that are supposed to become global top-$K$ items would actually be evicted during aggregation (Recall on Aggregation on light machines tends to be small). It can be concluded that the global top-$K$ selector favors items from heavy machines. Conversely, for underestimation sketches like Frequent, global top-$K$ selector tends to favors items from light machines. We argue that \unfair{} aggregation is unacceptable in many real-world applications since the global top-$K$ selector should not be partial to items from any machine.

2) One of the desired properties that \fairness{} brings is that the F1 Score of \fair{} algorithms, like our Double-Anonymous sketch, tends to be higher than \unfair{} algorithms. For example, for USS, local top-$K$ candidates in heavy machines tend to be highly overestimated, so even if an item in heavy machines is low in real frequency, its estimated frequency is still high enough to be falsely selected as a global top-$K$ item. With items in heavy machines falsely selected as global top-$K$ items and items in light machines ignored, the F1 Score of USS becomes unacceptably low when skewness is large.

3) Our approach is generic: we can make \textit{any} top-$K$ algorithm \fair{} simply by applying the Double-Anonymous sketch to this top-$K$ algorithm. Meanwhile, the F1 Score is also much improved because our approach is \fair{} in global top-$K$ aggregation.
}

\bbb{5.4.4 Other Baseline Algorithms}
 \\

\zyk{
\bbb{Comparison algorithms}:
%
In this section, we compare two other baseline algorithms designed for skewed data streams: algorithms based on global sampling and algorithms based on weighting.
%
For sampling algorithms, we use the same sampling rate for each data stream to sample items and send them to the global top-$K$ selector.
%
On the global top-$K$ selector, we use sketch data structures or directly use deterministic data structures (\eg{}, maps) to find global top-$K$ items in the sampled data stream.
%
For weighted algorithms, we maintain sketch data structures of different sizes on different machines according to the number of items contained in the data stream.
%
Specifically, if the data stream on the heavy machine contains 10 times as many items as that on the light machine, the sketch size on the heavy machine is set to be 10 times as large as that on the light machine.
}

\zyk{
\bbb{DA sketch \vs{} weighted algorithms (Figure \ref{fig:global_topk})}:
%
\hypertarget{link:exp_cmp}{We} compare weighted USS, weighted Waving, and weighted Ours+RA.
%
As shown in Figure \ref{subfig:global_topk:bias}, for weighted USS and weighted Waving, their overestimation on heavy machines is reduced, but their overestimation on light machines is significantly increased.
%
This is due to the non-linear relationship between their overestimation and the size of the data stream.
%
However, as shown in Figures \ref{subfig:global_topk:f1}, \ref{subfig:global_topk:small}, and \ref{subfig:global_topk:large}, weighting can indeed improve the performance of USS and Waving, especially when the distribution is particularly skewed.
%
Specifically, when $r=0.5$, the F1 score of weighted USS is 57.9\%, that of weighted Waving is 96.4\%, and that of weighted Ours+RA is 99.0\%.
}

\zyk{
\bbb{DA sketch \vs{} sampling algorithms (Table \ref{table:exp_sampling})}:
%
\hypertarget{link:exp_samp}{We} compare with the sampling algorithms using different sampling rates and different global data structures on global top-$K$ selectors.
%
The experimental results show that higher sampling rate means higher accuracy, but the performance of the sampling algorithm using 0.1 sampling rate and precise global data structure is still inferior to Ours+RA.
%
Furthermore, using a sampling algorithm with a rate of $p=0.1$, in total all machines need to transmit 8MB of data to the global top-$K$ selector;
%
using a sampling algorithm with a rate of $p=0.02$, all machines need to transmit 1.6MB of data.
%
By contrast, using Ours+RA, all machines only need to transmit $100\times15KB=1.5MB$ of data.
}

\begin{table}[!ht]
    \setlength{\abovecaptionskip}{-0.0cm}
    \setlength{\belowcaptionskip}{-0.0cm}
\centering
    \begin{tabular}{|c|c|c|}
        \hline
        Algorithms & F1 Score & ARE \\ \hline
        Sampling ($p=0.02$) + Precise & $85.8\%$ & $0.1234$ \\ \hline
        Sampling ($p = 0.1$) + Precise & $94.3\%$ & $0.0576$\\ \hline
        Sampling ($p = 0.02$) + RA & $68.3\%$ & $0.1367$ \\ \hline
        Sampling ($p = 0.1$) + RA & $73.4\%$ & $0.0958$ \\ \hline
        Ours + RA ($r = 0.5$) & $98.0\%$ & $0.0069$ \\ \hline
    \end{tabular}
    \caption{\revise{Comparisons between the sampling approach and our approach, where "precise" indicates that we use a deterministic algorithm to precisely record every sampled item.}}
    %\hwc{Remark: The reason why sampling + RA fails to achieve a satisfying F1 score is that the sampling process significantly reduces the skewness of the data stream, making the Top-$K$ item less distinguishable.} % sampling让数据流更"平"了, 使得top-K可分辨性更差, 优等生和差生更接近.
    \label{table:exp_sampling}
\end{table}

\zyk{
\ppp{Analysis}:
%
\hypertarget{link:disc_cmp}{For} the two comparison algorithms, the sampling algorithms are \fair{}, and the weighted algorithms can indeed improve the performance.
%
However, our algorithm still shows its superiority over the two algorithms.
%
In addition, there is another artificial weighted algorithm: manually correct the overestimation or underestimation of reported top-$K$ items from different data streams.
%
However, as shown in Section 5.4.2, the overestimation and underestimation of different algorithms are not consistent.
%
On the one hand, this algorithm is difficult to practice, and on the other hand, it cannot achieve the exact \fairness{}.
}

==> SIGMOD21/hwc/local_topk.tex <==
\presub
\subsection{Experiments on Local Top-$K$}
\label{sec:local_topk}
\postsub


\ppp{Application Description}: We first conduct experiments on finding local top-$K$ items and compare the Double-Anonymous sketch with prior art mentioned in \ref{sec:experimental-setup}. We use ARE, F1 Score, and Zero Error rate for evaluation.
\remove{
Since the Double-Anonymous sketch could provide not only unbiased estimation but also underestimation and overestimation, we also provide ARE results on both tasks and make a comparison with prior art.}
We also compare the performance of our three versions, \ie, the basic version, the Hot Panning Version, and the Early Freezing Version, and show how hot panning and early freezing improve the performance of our approach.

\remove{
\ppp{Experimental Settings}: In this experiment, we use both the CAIDA dataset and the synthetic dataset for our experiments. We set $K=1000$, and range the memory size from $100$KB to $500$KB for all sketches to see how different sketches perform in different amounts of memory. For underestimation and overestimation experiments, since prior art could provide only one type of frequency estimation method, we just use their default frequency estimation: the main purpose is to verify that the Double-Anonymous sketch performs well in underestimation and overestimation tasks.
}

\update{
\ppp{Experimental Settings}: In this experiment, we use the CAIDA dataset for our experiments. We set $K=1000$, and range the memory size from $100$KB to $500$KB for all sketches to see how different sketches perform in different amounts of memory.
}

\ppp{ARE (Figure \ref{subfig:local_topk:caida-ARE})}: 
%
Results show that our approach achieves much more accurate unbiased frequency estimation thanks to the hot panning and early freezing technique. When $M=100$KB, our approach is around $500$-$1000$ times more accurate than USS, SS, and Frequent and around $50$-$100$ times more accurate than Waving on the CAIDA dataset.

\ppp{F1 Score (Figure \ref{subfig:local_topk:caida-F1})}: 
%
When applying RA to our approach, the Double-Anonymous sketch achieves sufficiently high F1 Score ($\ge 95\%$) even when memory is extremely tight. 
%
This is because for the Double-Anonymous sketch, local top-$K$ items' selection is determined by only the replacement policy, and RA itself is accurate in selecting local top-$K$ items. 
%
In contrast, Frequent, USS, and SS are much more inaccurate in finding top-$K$ items. The discussion will be further elaborated in section \ref{sec:global_topk_balanced}.

\ppp{Zero Error Rate (Figure \ref{subfig:local_topk:zero_error_rate})}:
%
We demonstrate the proportion of items of which we are confident that frequency estimation error is guaranteed to be 0 (as denoted by zero error rate).
%
We could determine this because $C_{freezing} = 0$ indicates that such item has never been evicted from the Top-$K$ part throughout the process. 
%
The results show that our approach achieves a zero error rate greater than $40\%$ when memory is as tight as $100$KB, and greater than $72\%$ when $M=500$KB.
%
The results suggest that for the majority of items, our algorithm could tell with $100\%$ confidence that their estimated frequencies are perfectly accurate, which is useful in practice.


\ppp{Comparison between the three versions (Figure \ref{subfig:local_topk:three-version-are})}:
%
We find that both the hot panning and early freezing significantly improve the accuracy of our unbiased frequency estimation. 
%
On average, the final version --- the early freezing version is approximately 66 times more accurate than the first version --- the basic version and approximately 10 times more accurate than the second version --- the hot panning version.


\remove{
\ppp{ARE for Overestimation and Underestimation (Figure \ref{subfig:overestimate}) - \ref{subfig:underestimate}}: To demonstrate the accuracy of our algorithm on these two tasks, we compare our results with prior works with their respective frequency estimation querying method. We find that our approach could also provide accurate overestimation and underestimation for local top-$K$ items. Specifically, for overestimation, our approach achieves around 150 times lower ARE than Frequent, USS, and SS and 30 times lower ARE than Waving. 
For underestimation, our approach achieves around 100 times lower ARE than Frequent, USS, and SS and 20 times lower ARE than Waving.
Therefore, we conclude that our approach provides accurate underestimation, overestimation, and unbiased estimation simultaneously, which is useful for real-world application.
}

==> SIGMOD21/hwc/over_under_est.tex <==
%% need to be revised.
\presub
\subsection{Experiments on Overestimation and Underestimation}
\label{sec:experiment-overunderestimation}
\postsub


\ppp{Application Description}:
Besides unbiased estimation, \abbrev could also provide heavy hitters with one-side frequency estimation error: the estimated frequency is always an overestimation / underestimation of the real frequency. This one-side-error property is useful in many application scenarios. Here we apply \abbrev for heavy hitter detection using their overestimation and underestimation respectively. Specifically, we return all the items in the top-$K$ part with their overestimation / underestimation greater than a pre-defined threshold $\theta$. In comparison, we also apply USS and WavingSketch for finding heavy hitters and demonstrate the accurateness of our algorithm in this task.

\ppp{Experimental Settings}:
We conducted our experiments on the CAIDA dataset, and range the memory size from 100KB to 500KB. We set $\theta$ so that there are exactly $K=1000$ items whose real frequency $f_i$ is greater than $\theta$. All other settings are kept the same as the default settings described in section \ref{sec:experiment-param-settings}.

\ppp{Key results (Figure \ref{fig:overunderestimation})}:
First, we find that our algorithm achieves high enough F1 Score, even if memory size is tight. Specifically, when $M = 100$KB, F1 Scores of \abbrev+RA on both tasks are greater than $95\%$. Second, the underestimation and overestimation values of our algorithm are accurate. When $M = 200$KB, the ARE of \abbrev+RA on the underestimation and overestimation task is $0.006$ and $0.003$ respectively. This is $\ge 50 \times$ more accurate than USS, and $\ge 15 \times$ more accurate than WavingSketch.

% Apart from providing unbiased estimations, another critical function of UTF is to provide overestimation and underestimation for top-$K$ items, which are critical for many applications since they have one-sided error. Here we apply experimental settings in section \ref{sec:experiment-param-settings} and vary the memory size $M$ in this experiment.


% \ppp{Key Results (Figure \ref{fig:overunderest-are})}: We find that, for overestimation, ARE of all four UTF applications reduces to less than $\le 0.01$ when $M>200$KB, which is a relatively good score in the CAIDA dataset. For overestimation, The ARE of UTF applications is  $69.56$, $106.2$, $33.26$, and $26.65$ times lower than USS in average respectively. Besides, for underestimation, the ARE is $31.87$, $23.85$, $20.99$, and $16.07$ times lower than USS respectively.




\ppp{Analysis}: Our experimental results show that, \abbrev could provide not only accurate unbiased estimations but also accurate enough overestimation and underestimation for heavy hitter detection at the same time within a \textit{single} sketch. This property is desirable when putting UTF into practice.

% The facts that all the UTF applications achieve F1 Score close to 1 when $M \ge 200$KB, and that UTF applications achieve relatively low level of ARE, These indicate that UTF is suitable to be put into practice in senarios. %. It is worth pointing out that, if we compare the results of Figure \ref{fig:overunderest-are} with Figure \ref{subfig:ARE:CAIDA}, we would find that overestimation and underestimation are generally not as accurate as unbiased estimation but still accurate enough for real-world practice.



==> SIGMOD21/hwc/param_settings.tex <==
\presub
\subsection{Experiments on Parameter Settings}
\postsub
\label{subsec:Parameter Settings}


In order to find the optimal parameter settings for the Double-Anonymous sketch, we conduct experiments on finding local top-$K$ items and vary $\lambda$ and $\frac{M_{top-K}}{M}$ to see how AAE, ARE, F1 Score and Throughput change.  We set $M$ to be $100$KB, $\lambda$ to range from $1$ to $64$, and $\frac{M_{top-K}}{M}$ to range from $0.05$ to $0.95$. 


\ppp{Varying $\lambda$ (Figure \ref{subfig:varying-lambda-are}-\ref{subfig:varying-lambda-th})}: We find that, as $\lambda$ increases from 1 to 64, ARE of Our+RA and Ours+SS first decreases when $\lambda$ grows from $1$ to $8$ by $6.8$ times and $3.2$ times respectively and then remains steady. For Ours+HG and Ours+Freq, ARE keeps roughly steady. However, as $\lambda$ increases, the throughput of all Double-Anonymous sketch applications drops severely: on average, throughput when $\lambda=64$ is $2.3$ times smaller than throughput when $\lambda=1$. Therefore in practice, we choose $\lambda=8$ as the best setting.

\ppp{Varying $\frac{M_{top-K}}{M}$ (Figure \ref{subfig:varying-ratio_ARE}-\ref{subfig:varying-ratio_rc})}: We find that F1 scores grow as $\frac{M_{top-K}}{M}$ increases, since F1 scores are only determined by the top-$K$ part. However, we find that when $\frac{M_{top-K}}{M} \ge 0.55$, growth rate of F1 scores of all Double-Anonymous sketch applications becomes slow if $\frac{M_{top-K}}{M}$ continues to increase. In addition, in this experiment, $M=100$KB is tight, and if $M$ becomes larger, growth of F1 scores contributed by $\frac{M_{top-K}}{M}$ will become more negligible. Besides, Ours+HG and Ours+RA reach their respective minimal ARE score when $\frac{M_{top-K}}{M} \approx 0.55$ ($2.7$ and $1.8$ times smaller than when $\frac{M_{top-K}}{M} = 0.05$ and $2.5$ and $3.0$ times smaller than when $\frac{M_{top-K}}{M} = 0.95$), while Ours+Freq and Ours+SS reach their minimal ARE when $\frac{M_{top-K}}{M} \approx 0.75$. In practice, we choose $\frac{M_{top-K}}{M} = 0.55$ as the default parameter setting.


\zyk{
\ppp{Analysis}:
%
\hypertarget{link:disc_rep_3}{1)} Among the four replacement policies, Ours+RA and Ours+HG often have higher performance than Ours+Freq and Ours+SS.
%
Specifically, Ours+RA has more advantages in F1 score, while Ours+HG has more advantages in ARE.
%
Considering that Ours+RA has higher throughput, we recommend using Ours+RA in practice.
%
2) However, although Ours+Freq and Ours+SS are slightly inferior in accuracy, Freq and SS are famous for their formal and comprehensive error theories and error bounds.
%
Benefiting from their theories, we suggest that Ours+Freq and Ours+SS should be considered in scenarios where exact error guarantees are required.
}

==> SIGMOD21/hwc/setup.tex <==
\presub
\subsection{Experimental Setup}
\label{sec:experimental-setup}
\postsub


\remove{
\ppp{A. Implementation}:
We have implemented the Double-Anonymous sketch and all other algorithms in C++. We apply four replacement strategies to the Double-Anonymous sketch: Randomized Admission Policy (RA) \cite{rap}, SpaceSaving (SS) \cite{spacesaving}, Frequent (Freq) \cite{frequent} and HeavyGuardian (HG) \cite{heavyguardian}. 
%
We find in our experimental results that applying Randomized Admission Policy  yields the best results; therefore, we mainly demonstrate the experimental results of Double-Anonymous sketch + RA. We also demonstrate experiments for the other three strategies in section \label{subsec:Parameter Settings}.
%
We also compare our results with several state-of-the-art top-$K$ sketching algorithms: Frequent \cite{frequent}, SpaceSaving \cite{spacesaving}, Unbiased SpaceSaving \cite{unbiasedsketch} and WavingSketch \cite{li2020wavingsketch}.
%
Frequent tends to underestimate items' frequency, and SpaceSaving tends to overestimate items' frequency.
%
Both Unbiased SpaceSaving and WavingSketch achieve unbiasedness, but when considering only the selected top-$K$ items, they tend to overestimate items' frequency.
%
For WavingSketch, we use its unbiased frequency estimation method rather than the biased estimation method: 
%
preliminary results show that although biased estimation method achieves slightly lower frequency estimation error, unbiased estimation method achieves better \fairness{} in Section~\ref{sec:global_topk_imbalanced}.
%
All our experiments are repeatedly performed 10 times to ensure statistical stability.
%
Abbreviations used in our experiments are shown in table \ref{table:hwc:abbr}. Our source code is publicly available at Github \cite{opensource}. 
}

\update{
\ppp{A. Implementation}:
We have implemented the Double-Anonymous sketch (DA sketch) and all other algorithms in C++. 
%
We apply four replacement strategies to the DA sketch: Randomized Admission Policy (RA) \cite{rap}, SpaceSaving (SS) \cite{spacesaving}, Frequent (Freq) \cite{frequent} and HeavyGuardian (HG) \cite{heavyguardian}. 
%
We find in our experimental results that applying Randomized Admission Policy  yields the best results; therefore, we mainly demonstrate the experimental results of DA sketch + RA.
%
We also compare our results with several state-of-the-art top-$K$ sketching algorithms: Frequent \cite{frequent}, SpaceSaving \cite{spacesaving}, Unbiased SpaceSaving (USS) \cite{unbiasedsketch} and WavingSketch (Waving) \cite{li2020wavingsketch}.
%
All our experiments are repeatedly performed 10 times to ensure statistical stability.
%
Our source code is publicly available at Github \cite{opensource}. %
We conduct all our experiments on a machine with two 6-core processors (12 threads, Intel Xeon CPU E5-2620 @2 GHz) and 64 GB DRAM memory.
}


\remove{
\ppp{B. Computational Platform}:
We conduct all our experiments on a machine with two 6-core processors (12 threads, Intel Xeon CPU E5-2620 @2 GHz) and 64 GB DRAM memory. Each processor has three cache memory levels: one 32KB L1 data caches and one 32KB L1 instruction cache for each core, one 256KB L2 cache for each core, and one 15MB L3 cache shared by all cores.
}

\ppp{B. Datasets}: We use three real-world datasets and one synthetic dataset for our experiments. The details of the datasets are shown below:
\label{sec:experimental-setup-datasets}
%
1) IP Trace Dataset (CAIDA) \cite{caida}: The IP Trace Dataset consists of streams of anonymous IP traces collected by CAIDA in 2016. Each item is identified by its 13-byte "5-Tuple". We use the first 20M items for our experiments.
%
2) Web Page Dataset \cite{webdocs}: The Web page dataset is built from a collection of web pages downloaded from the website.
Each item is 4 bytes long.
%
3) Network Dataset \cite{net_dat}: The network dataset consists of users' posting history on the StackExchange website. 
%
4) Synthetic Dataset: We generated datasets following the Zip-f  distribution \cite{zipf}. Each dataset contains 32M items, and each item is 4 bytes long. Here we use the generated dataset with skewness=$0.6$.

\ppp{C. Metrics}:
\label{sec:exerimental-setup-metrics}

\ppp{1) Average Relative Error (ARE):} $\frac{1}{|\mathbf{\Psi}|} \sum_{e_i \in \mathbf{\Psi}}\frac{|f_i-\hat{f_i}|}{f_i}$,
where $f_i$ is the ground truth frequency of item $e_i$, $\hat{f_i}$ is its estimated frequency, and $\mathbf{\Psi}$ is the query set. 

\ppp{2) F1 Score:}
$\frac{2 * CR * PR}{CR + PR}$, where $PR$ (Precision rate) represents the proportion of the correctly selected items among all the selected items, and $CR$ (Recall rate) represents the proportion of the correctly selected items among all the real top-$K$ items. 

\ppp{3) Throughput:}
The number of operations (insertions) in million per second (Mops). It indicates the overall speed of insertion.

\ppp{4) Zero Error Rate:} The proportion of items selected by our sketch whose estimated frequency is guaranteed to be exactly the same as its ground truth frequency. 

\ppp{5) Relative Bias:}
This metric is used in section \ref{sec:global_topk_imbalanced}.
%
For the local sketch $i$, the relative bias is defined $\frac{\sum_{e_j \in \mathbf{\Psi}}\hat{f_j}}{\sum_{e_j \in \mathbf{\Psi}}f_j} $, where $\Psi$ is the set of items that local sketch $i$ returns as the local top-$K$ items.

\ppp{6) Recall on Aggregation: $\frac{||\{(\mathcal{\hat{T}}_i \cap \mathcal{T}) \cap \mathcal{\hat{T}}\}||}{||\{\mathcal{\hat{T}}_i \cap \mathcal{T}\}||}$} for local sketch $i$, where $\mathcal{T}$ denotes the set of global top-$K$ items, $\mathcal{\hat{T}}$ denotes the set of \textit{predicted} global top-$K$ items (after aggregation), and $\mathcal{\hat{T}}_i$ denotes the selected local top-$K$ items from sketch $i$.

\ppp{D. Common Settings:} 
%
Let $M$ denote the total amount of memory allocated to the sketches, $M_{top-K}$ denote the amount of memory allocated to the top-$K$ part for the DA sketch, $K$ denote that we query the top-$K$ frequent items, and $\lambda$ denotes the number of cells in each bucket of the top-$K$ part. 
%
For the DA sketch, we set $\lambda=8$, $\frac{M_{top-K}}{M}=0.55$ in order to maximize the overall performance.
5
For DA sketch, the size of count part's buckets in the Hot Panning version and the Early Freezing is set to be $2$ bytes; 
%
while for the basic version, the size of count part's buckets is set to be $4$ bytes. 
%
All other parameters of the baseline top-$K$ algorithms are set according to the recommendations of their authors. 

\ppp{Settings for Figure \ref{subfig:intro-internal-unfair} in Section \ref{intro:prior-works}}:
\label{subsec:intro-settings-1}
We perform the finding local top-$K$ tasks on CAIDA dataset for both USS and Waving, for $1000$ times each. 
%
Memory size is set to be $100$KB, and $K$ is set to be $1000$. 
%
After insertion, we calculate the total (signed) error for both the selected Top-$K$ items and items that are not selected. 
%
We average the results over the $1000$ times of experiments. 

\ppp{Settings for Figure \ref{subfig:intro-recall-top-1} in Section \ref{intro:prior-works}}: 
\label{subsec:intro-settings-2}
We conduct experiments on the Synthetic Dataset. We generate the dataset so that the global Top-1 item is always in the light stream. 
%
We set $N=100, K=50$ and range skewness from $0.1$ to $0.4$. 
%
We only allocate an extremely small amount of memory for both USS and Ours+SS, such that they could only store $K=50$ local top-$K$ candidates for each distributed sketch ($3.8$KB for USS and $1.4$KB for Ours+SS). 
%
In such an extremely small amount of memory and high skewness, the estimated frequency of the selected local top-$K$ items in the heavy stream would even be greater than the frequency of the global Top-1 item in the light stream. Therefore, the global Top-1 may be ignored when skewness is high.

==> SIGMOD21/hwc/verify_bound.tex <==
%% Need to be revised!

\subsection{Validation of the Theoretical Variance Bound}
\label{sec:experiment-bound-verification}

As shown in Figure \ref{fig:bound}, we conduct experiments to demonstrate the loose and tight variance bound derived in Theorem \ref{theo:bound}, and the real experimental value of the basic version and the optimized version. Here we keep the size and strategy of the top-k part fixed and gradually increase $w$. We conduct multiple times of experiments to derive the experimental values. Please note that the loose bound is unrelated to top-k strategy, while the tight bound is related.The tight variance bound is always just greater than the experimental results of the basic version, which verifies the correctness of theorem \ref{theo:bound}. Interestingly, the real bound values of the basic version are extremely close to the tight bound, indicating the tightness of the tight bound. Experimental results also show that there are big gaps between the loose bound and the tight bound, and between the real value of the basic version and the optimized version.

==> SIGMOD21/zyk/exp_veri.tex <==

To verify the correctness of Lemma~\ref{lem:error} and Theorem~\ref{theo:freezing_bound}, we show two kinds of variance bound.
%
Lemma~\ref{lem:error} provides a $\mathcal{P}$-independent loss bound, and an $\mathcal{R}$-dependent tight bound.
%
We use SpaceSaving and Randomized Admission Policy as the strategy $\mathcal{P}$, and vary the length $w$ of the count part.
%
%
As shown in Figure~\ref{fig:bound}, we plot the loose upper bounds, the tight upper bounds, 
%
and the sample variances of the hot panning version and the early freezing version.
%
%
It can be found that the bounds of variances are always greater than the sample variances of the hot panning version,
%
and then greater than the sample variances of the early freezing version, which verifies our theorems and shows the benefits of Early Freezing.
%
%
It is worth noting two points:
%
1) The tight bounds are extremely close to the sample variances, which indicates our bounds are accurate.
%
2) Panning hot items to reduce the redundancy is beneficial to reduce variance, 
%
and the strategy of finding top-$K$ frequent items more accurately has a smaller variance.



==> SIGMOD21/zyk/lemma_iden.tex <==
\begin{lemma}
\label{lem:iden}
%
%
Given a data stream $\mathcal{S}$ and a process $\mathcal{R}=\{s_1,\cdots,s_m\}$, 
%
for any item $i\in\mathcal{U}$ and any time $1\leqslant j\leqslant m$, there is 
%
\begin{align}
f^{T}_{(i,j)}+f^{S}_{(i,j)}=f_{(i,j)}.
\end{align}
%
\end{lemma}


\preproof \begin{proof}
\label{prf:iden}





For any item $i$, we consider the change of its state $s_{(i,j-1)}$ at time $j$.
%
There are two cases at time $j$, \ie, $e_j=i$ or $e_j\ne i$.
%
We analyze the change of state $s_{(i,j)}$ in each case in detail below.




\noindent\textbf{Cases 1:} 
%
$e_j=i$, and the $C_r$ of item $i$ $\left(f^{T}_{(i,j-1)}\right)$ becomes $C_r'$ after time $j$ $\left(f^{T}_{(i,j)}\right)$.

In this case, we increase the frequency of item $i$ recorded in the sketch part by $\left(C_r-C_r'\right)+1$.
%
Thus we have
%
\begin{align}
\left\{
\begin{aligned}
f^{T}_{(i,j)}&=&f^{T}_{(i,j-1)}+\left(C_r'-C_r\right)\\
f^{S}_{(i,j)}&=&f^{S}_{(i,j-1)}+\left(C_r-C_r'\right)+1
\end{aligned}
\right.\
\end{align}





\noindent\textbf{Cases 2:} 
%
$e_j\neq i$, and the $C_r$ of item $i$ $\left(f^{T}_{(i,j-1)}\right)$ becomes $C_r'$ after time $j$ $\left(f^{T}_{(i,j)}\right)$.

In this case, we increase the frequency of item $i$ recorded in the sketch part by $\left(C_r-C_r'\right)$.
%
Thus we have
%
\begin{align}
\left\{
\begin{aligned}
f^{T}_{(i,j)}&=&f^{T}_{(i,j-1)}+\left(C_r'-C_r\right)\\
f^{S}_{(i,j)}&=&f^{S}_{(i,j-1)}+\left(C_r-C_r'\right)
\end{aligned}
\right.
\end{align}

Considering both cases, we can find 
%
%
\begin{align}
    \left(f^{T}_{(i,k)}+f^{S}_{(i,k)}\right)
    -
    \left(f^{T}_{(i,k-1)}+f^{S}_{(i,k-1)}\right)
    =
    1_{\{e_k=i\}}.
\end{align}
%
Since the above formula holds for any time $k$, by summing $k$ from $1$ to $j$, we can get
%
\begin{align}
&
    f^{T}_{(i,j)}+f^{S}_{(i,j)}
\notag\\
=&  \sum_{k=1}^j \left(
    \left(f^{T}_{(i,k)}+f^{S}_{(i,k)}\right)
    -
    \left(f^{T}_{(i,k-1)}+f^{S}_{(i,k-1)}\right)
    \right)
\notag\\
=&  \sum_{k=1}^j 1_{\{e_k=i\}} = f_{(i,j)}.
\end{align}

\end{proof} \postproof

==> SIGMOD21/zyk/lemma_mono.tex <==
\begin{lemma}
\label{lem:mono}
%
%
Given a data stream $\mathcal{S}$ and a process $\mathcal{R}=\{s_1,\cdots,s_m\}$, 
%
%
for any item $i$ and any time $j$, there is
%
\begin{align}
f^{S}_{(i,j-1)} \leqslant f^{S}_{(i,j)} \leqslant f_{(i,j)}.
\end{align}

\end{lemma}


\preproof \begin{proof}
\label{prf:mono}



By definition, $C_r$ is the frequency of an item recorded by the top-$K$ part, so we can naturally get $C_r\geqslant 0$.
%
In other words, for any item $i$ and time $j$, we have $f^{T}_{(i, j)}\geqslant 0$.
%
By lemma \ref{lem:iden}, we know that for any item $i$ and time $j$, there is
%
\begin{align}
f^{T}_{(i,j)}+f^{S}_{(i,j)} = f_{(i,j)}.
\end{align}
%
So according to $f^{T}_{(i, j)}\geqslant 0$, we can get $f^{S}_{(i,j)} \leqslant f_{(i,j)}$ immediately.




To prove the monotonicity of $f^{T}_{(i,j)}$, we discuss the change of $C_r$ and $f^{T}_{(i,j)}$ in 2 cases defined in Proof~\ref{lem:iden}.
%
\begin{itemize}[leftmargin=*]
    \item In the case 1, since $C_r'=C_r+1$ (item $i$ is recorded in the top-$K$ part after time $j$) or $C_r'=0$ (item $i$ is not recorded in the top-$K$ part after time $j$), then $\left(C_r-C_r'\right)+1\geqslant 0$, and $f^{T}_{(i,j)} \geqslant f^{T}_{(i,j-1)}$ holds.
    %
    \item In the case 2, since $C_r'=C_r$ (item $i$ is still recorded in the top-$K$ part after time $j$) or $C_r'=0$ (item $i$ is not recorded in the top-$K$ part after time $j$), then $\left(C_r-C_r'\right)\geqslant 0$, and $f^{T}_{(i,j)} \geqslant f^{T}_{(i,j-1)}$ holds.
\end{itemize}
%
To sum up, we have for any item $i$ and any time $j$, the following formula always holds.
%
\begin{align}
    f^{S}_{(i,j-1)} \leqslant f^{S}_{(i,j)} \leqslant f_{(i,j)}.
\end{align}

\end{proof} \postproof

==> SIGMOD21/zyk/other_math.tex <==
Let the random variable 
\begin{align}
Y_{i,i'}
=
\sum_{k=1}^d\sum_{k'=1}^d\sum_{j=1}^{f^{(3)}_{i',m}}
I_{i,k,i',k'}\cdot I_{i',j,k'}
.
\end{align}
%
Since $f^{(3)}_{(i,m)}$ is a constant under a given $\mathcal{R}$, and $Y_{i,i'}$ and $Y_{i,i''}$ are independent when $i'\neq i''$, we have
\begin{align}
    D\left(\sum_{k=1}^d X_{(i,k)}~|~\mathcal{R}\right)
    =
    \sum_{i'\neq i} D\left(Y_{i,i'}~|~\mathcal{R}\right).
\end{align}





Next we analyze the variance of the random variable $Y_{i,i'}$.
%
We rewrite $Y_{i,i'}$ as follows.
%
\begin{align}
Y_{i,i'}
=&
\sum_{k'=1}^d
\left(\sum_{k=1}^d I_{i,k,i',k'}\right)
\left(\sum_{j=1}^{f^{(3)}_{i',m}} I_{i',j,k'}\right)
\notag\\
=&
\sum_{k'=1}^d N_{i,i',k'}\cdot S_{i',k'}
.
\end{align}
%
Where $N_{i,i',k'}$ indicates how many $k$ make $h_k(e_i)$ and $h_{k'}(e_{i'})$ equal, $S_{i',k'}$ indicates how many times the occurrence of item $e_{i'}$ chooses the $h_{k'}(e_{i'})$-th counter to add $1$.
%
Specifically,
%
\begin{align}
    \left\{
    \begin{aligned}
    N_{i,i',k'} &=& \sum_{k=1}^d I_{i,k,i',k'}
    \\
    S_{i',k'} &=& \sum_{j=1}^{f^{(3)}_{i',m}} I_{i',j,k'}
    \end{aligned}
    \right.
\end{align}
%
Note that when $k'\neq k''$, random variables $N_{i,i',k'}$ and $N_{i,i',k''}$, $N_{i,i',k'}$ and $S_{i',k'}$ are independent of each other.



We need to calculate the first moment of $Y_{i,i'}$.
%
\begin{align}
E\left(Y_{i,i'}~|~\mathcal{R}\right)
=&
E\left(\sum_{k'=1}^d N_{i,i',k'}\cdot S_{i',k'}~|~\mathcal{R}\right)
\notag\\
=&
\sum_{k=1}^d
E\left(\sum_{k'=1}^d I_{i,k,i',k'}~|~\mathcal{R}\right)
E\left(\sum_{j=1}^{f^{(3)}_{i',m}} I_{i',j,k'}~|~\mathcal{R}\right)
\notag\\
=&
d\cdot \left(d\cdot \frac{1}{w}\right) \cdot \left(f^{(3)}_{i',m}\cdot \frac{1}{d}\right)
\notag\\
=&
\frac{d\cdot f^{(3)}_{i',m}}{w}.
\end{align}
We also need to calculate the second moment of $Y_{i,i'}$.
\begin{align}
&
E\left(Y_{i,i'}^2~|~\mathcal{R}\right)
\notag\\
=&
E\left(
\left(
\sum_{k'=1}^d N_{i,i',k'}\cdot S_{i',k'}
\right)^2
~|~\mathcal{R}
\right)
\notag\\
=&
\sum_{k'=1}^{d}\sum_{k''=1}^d
E\left(
N_{i,i',k'}\cdot N_{i,i',k''}\cdot S_{i',k'}\cdot S_{i',k''}
~|~\mathcal{R}\right)
\notag\\
=&
\sum_{k'=1}^{d}
E\left(
N_{i,i',k'}^2
~|~\mathcal{R}\right)
E\left(
S_{i',k'}^2
~|~\mathcal{R}\right)
\notag\\
+&
\sum_{k'\neq k''}
E\left(
N_{i,i',k'}
~|~\mathcal{R}\right)
E\left(
N_{i,i',k''}\
~|~\mathcal{R}\right)
E\left(
S_{i',k'}\cdot S_{i',k''}
~|~\mathcal{R}\right)
.
\end{align}
%
Since we have
%
\begin{align}
&
E\left(
N_{i,i',k'}^2
~|~\mathcal{R}\right)
\notag\\
=&
E\left(
\left(
\sum_{k=1}^d I_{i,k,i',k'}
\right)^2
~|~\mathcal{R}\right)
\notag\\
=&
\sum_{k=1}^d
E\left(
I_{i,k,i',k'}^2
~|~\mathcal{R}\right)
+
\sum_{k\neq k''}
E\left(
I_{i,k,i',k'}\cdot I_{i,k'',i',k'}
~|~\mathcal{R}\right)
\notag\\
=&
d\cdot\frac{1}{w}+d\cdot (d-1)\cdot \frac{1}{w^2}
\notag\\
=&
\frac{d\cdot(d+w-1)}{w^2}
.
\end{align}
%
And
%
\begin{align}
&
E\left(
S_{i',k'}^2
~|~\mathcal{R}\right)
\notag\\
=&
E\left(
\left(
\sum_{j=1}^{f^{(3)}_{i',m}} I_{i',j,k'}
\right)^2
~|~\mathcal{R}\right)
\notag\\
=&
\sum_{j=1}^{f^{(3)}_{i',m}}
E\left(
I_{i',j,k'}^2
~|~\mathcal{R}\right)
+
\sum_{j\neq j'}
E\left(
I_{i',j,k'}\cdot I_{i',j',k'}
~|~\mathcal{R}\right)
\notag\\
=&
f^{(3)}_{i',m}\cdot\frac{1}{d}
+
f^{(3)}_{i',m}\cdot (f^{(3)}_{i',m}-1)\cdot \frac{1}{d^2}
\notag\\
=&
\frac{f^{(3)}_{i',m}\cdot(f^{(3)}_{i',m}+d-1)}{d^2}
.
\end{align}
%
And
%
\begin{align}
&
E\left(
S_{i',k'}\cdot S_{i',k''}
~|~\mathcal{R}\right)
\notag\\
=&
E\left(
\left(
\sum_{j=1}^{f^{(3)}_{i',m}} I_{i',j,k'}
\right)
\cdot
\left(
\sum_{j‘=1}^{f^{(3)}_{i',m}} I_{i',j’,k'‘}
\right)
~|~\mathcal{R}\right)
\notag\\
=&
\sum_{j=1}^{f^{(3)}_{i',m}}
E\left(
I_{i',j,k'}\cdot I_{i',j,k''}
~|~\mathcal{R}\right)
+
\sum_{j\neq j'}
E\left(
I_{i',j,k'}\cdot I_{i',j',k''}
~|~\mathcal{R}\right)
\notag\\
=&
f^{(3)}_{i',m}\cdot (f^{(3)}_{i',m}-1)\cdot \frac{1}{d^2}
.
\end{align}
We can get
\begin{align}
&
E\left(Y_{i,i'}^2~|~\mathcal{R}\right)
\notag\\
=&
d
\cdot
\left(
\frac{d\cdot(d+w-1)}{w^2}
\right)
\cdot
\left(
\frac{f^{(3)}_{i',m}\cdot(f^{(3)}_{i',m}+d-1)}{d^2}
\right)
\notag\\
+&
d\cdot (d-1)
\cdot
\left(
\frac{d}{w}
\right)
\cdot
\left(
\frac{d}{w}
\right)
\cdot
\left(
f^{(3)}_{i',m}\cdot (f^{(3)}_{i',m}-1)\cdot \frac{1}{d^2}
\right)
\notag\\
=&
\frac{(d+w-1)\cdot f^{(3)}_{i',m}\cdot (f^{(3)}_{i',m}+d-1)}{w^2}
\notag\\
+&
\frac{d\cdot(d-1)\cdot f^{(3)}_{i',m}\cdot (f^{(3)}_{i',m}-1)}{w^2}
\notag\\
\end{align}
%
According to the formula of variance, we can get
\begin{align}
D\left(Y_{i,i'}~|~\mathcal{R}\right)
=&E\left(Y_{i,i'}^2~|~\mathcal{R}\right)-E\left(Y_{i,i'}~|~\mathcal{R}\right)^2
\notag\\
=&
\frac{(d+w-1)\cdot f^{(3)}_{i',m}\cdot (f^{(3)}_{i',m}+d-1)}{w^2}
\notag\\
+&
\frac{d\cdot(d-1)\cdot f^{(3)}_{i',m}\cdot (f^{(3)}_{i',m}-1)}{w^2}
\notag\\
-&
\left(\frac{d\cdot f^{(3)}_{i',m}}{w}\right)^2.
\notag\\
\leqslant&
\frac{f^{(3)}_{i',m}\cdot (f^{(3)}_{i',m}+d)}{w}
.
\end{align}
%
According to Lemma \ref{lem:mono}, we have
\begin{align}
    D\left(Y_{i,i'}~|~\mathcal{R}\right)
    \leqslant 
    \frac{f_{i'}^2+d\cdot f_{i'}}{w}.
\end{align}
%
By summing up $D\left(Y_{i,i'}~|~\mathcal{R}\right)$, we can get
\begin{align}
     D\left(\sum_{k=1}^d X_{(i,k)}~|~\mathcal{R}\right)
     \leqslant&
     \sum_{i'=1}^n D\left(Y_{i,i'}~|~\mathcal{R}\right)
     \notag\\
     \leqslant&
     \sum_{i'=1}^n \frac{f_{i'}^2+d\cdot f_{i'}}{w}
     \notag\\
     =&
     \frac{\sum_{i'=1}^n f_{i'}^2+d\cdot \sum_{i'=1}^n f_{i'}}{w}.
\end{align}

==> SIGMOD21/zyk/preliminary.tex <==
\remove{
Since we only focus on a single data stream in this section, we decided to use some symbols that are simpler than the definitions in Section \ref{related::pre} to describe theorems and proofs more intuitively.
%
We first define the concepts of data stream and frequency.
%
Let $\mathcal{S}=\{e_1,e_2,\cdots,e_m\}$ be a data stream contains $m$ items, 
%
where $e_j \in \{1,2,\cdots,n\}$, and we say that item $e_j$ appears at time $j$.
%
Let $f_{(i,j)}=\sum_{k=1}^j 1_{\{e_k=i\}}$ be the frequency of item $i$ at time $j$, and let $f_i=f_{(i,m)}$ be the frequency of the item $i$ in data stream $\mathcal{S}$.
}


We then define the state $s_{(k,t)}$ of the Double-Anonymous sketch on data stream $\mathcal{S}_k$ at time $t$ as $s_{(k,t)} = \{s_{(k,1,t)}, \cdots, s_{(k,n_k,t)}\}$, where $ s_{(k,i,t)}= \langle f_{T(k,i,t)},f_{S(k,i,t)} \rangle $.
%
In general, let $f_{T(k,i,t)}$ be the frequency of item $u_{(k,i)}$ recorded in the top-$K$ part at time $t$, and let $f_{S(k,i,t)}$ be the frequency of item $i$ recorded in the count part at time $t$.
%
In particular, if item $u_{(k,i)}$ is not recorded in the top-$K$ part at time $j$, let $f_{T(k,i,t)}=0$.




Given a data stream $\mathcal{S}_k$, let a \textit{sketching process} $\mathcal{R}$ be a sequence of states of the Double-Anonymous sketch at each time, \ie, $\mathcal{R}=\{s_{(k,1)},s_{(k,2)},\cdots,s_{(k,m_k)}\}$.
%
The replacement policy $\mathcal{P}$ determines the distribution of the sketching process, \ie, $\mathcal{R}\sim\mathcal{P}(\mathcal{S}_k)$.

==> SIGMOD21/zyk/theorem_bound.tex <==

\begin{theorem}[Error Bound]
\label{theo:bound}


Given a data stream $\mathcal{S}$, for any strategy $\mathcal{P}$ and any item $i$, let $\hat{f_i}$ be the unbiased estimation of $f_i$ given by UTF, then we have
%
\begin{align}
    \Pr\left(\left|~\hat{f_i}-f_i~\right|
    \geqslant\varepsilon\right) \leqslant
    \frac{1}{\varepsilon^2\cdot d\cdot (w-1)} \cdot
    \left(\sum_{i'=1}^{n} f_{i'}^2\right).
\end{align}
\end{theorem}

\preproof \begin{proof}
\label{prf:bound}



According to Theorem \ref{theo:unbias}, we know that there is
%
\begin{align}
    E\left(\hat{f_i}\right) = f_i
\end{align}
%
%
According to Theorem \ref{theo:error}, we know that there is
%
\begin{align}
    D\left(\hat{f_i}\right) \leqslant
    \frac{1}{d\cdot (w-1)} \cdot
    \left(\sum_{i'=1}^{n} f_{i'}^2\right).
\end{align}
%
%
Using Chebyshev inequality, we can get
%
\begin{align}
    \Pr\left(\left|~\hat{f_i}-f_i~\right|
    \geqslant\varepsilon\right)
=&
    \Pr\left(\left(\hat{f_i} - E\left(\hat{f_i}\right)\right)^2
    \geqslant\varepsilon^2\right)
\notag\\
\leqslant&
    \frac{1}{\varepsilon^2}\cdot D\left(\hat{f_i}\right)
\notag\\
\leqslant&
    \frac{1}{\varepsilon^2\cdot d\cdot (w-1)} \cdot
    \left(\sum_{i'=1}^{n} f_{i'}^2\right).
\end{align}
\postproof \end{proof}


\begin{theorem}[Error Bound, Overestimation]
\label{theo:bound}


Given a data stream $\mathcal{S}$, for any strategy $\mathcal{P}$ and any item $i$, let $\overline{f_i}$ be the overestimation of $f_i$ given by UTF, then we have
%
\begin{align}
    \Pr\left(\overline{f_i}-f_i\geqslant\varepsilon\right) \leqslant
    \left(\frac{1}{\varepsilon\cdot w} \cdot
    \left(\sum_{i'=1}^{n} f_{i'}\right)\right)^{d}.
\end{align}
\end{theorem}

\preproof \begin{proof}
\label{prf:bound}

We first prove that the following inequality holds for any process $\mathcal{R}$ of strategy $\mathcal{P}$, for any item $i$ and random variable $X_{(i, k)}$.
\begin{align}
    E\left(X_{(i,k)}-f^{S}_{(i,m)}~|~\mathcal{R}\right) \leqslant
    \frac{1}{w}\cdot\left(\sum_{i'=1}^n f_{i'}\right).
\end{align}

Recalling our definition of $X_{(i,k)}$ in Formula~\ref{form:rv}, we have
\begin{align}
    X_{(i,k)}-f^{S}_{(i,m)}=\sum_{i'=1,i'\ne i}^{n}
    \left(I_{(i,i',k)}\cdot f_{(i',m)}\right).
\end{align}
According to the linearity of expectation, we have
\begin{align}
    E\left(X_{(i,k)}-f^{S}_{(i,m)}~|~\mathcal{R}\right) 
    =&
    \sum_{i'=1,i'\ne i}^{n}
    \left(E\left(I_{(i,i',k)}~|~\mathcal{R}\right) \cdot
    f^{S}_{(i',m)}\right)
    \notag\\
    =&
    \sum_{i'=1,i'\ne i}^{n}
    \left(\frac{1}{w} \cdot f^{S}_{(i',m)}\right)
\leqslant
    \frac{1}{w}\cdot\left(\sum_{i'=1}^{n} f_{i'}\right).
\end{align}
Then, using the total expectation formula, we have
\begin{align}
    E\left(X_{(i,k)}-f^{S}_{(i,m)}\right) \leqslant
    \frac{1}{w}\cdot\left(\sum_{i'=1}^{n} f_{i'}\right).
\end{align}

Using Markov inequality, we have
\begin{align}
    \Pr\left(X_{(i,k)}-f^{S}_{(i,m)} \geqslant\epsilon\right) 
\leqslant&
    \frac{1}{\epsilon} \cdot E\left(X_{(i,k)}-f^{S}_{(i,m)}\right)
\notag\\
\leqslant&
    \frac{1}{\epsilon\cdot w}\cdot\left(\sum_{i'=1}^{n} f_{i'}\right).
\end{align}
Since we use $f^{T}_{(i,m)}+\left(\min_{k=1}^{d} X_{(i,k)} \right)$ as the overestimation $\overline{f_i}$, and the random variables $X_{(i,k)}$ are independent of each other, we have
\begin{align}
&
    \Pr\left(\overline{f_i}-f_i\geqslant\varepsilon\right)
\notag\\
=&
    \Pr\left(
    \left(f^{T}_{(i,m)} +
    \left(\min_{k=1}^{d} X_{(i,k)} \right)\right) - 
    \left(f^{T}_{(i,m)}+f^{S}_{(i,m)}\right)
    \geqslant\varepsilon\right)
\notag\\
=&
    \Pr\left(
    \left(\min_{k=1}^{d} X_{(i,k)}\right)-f^{S}_{(i,m)}
    \geqslant\varepsilon\right)
\notag\\
=&
    \prod_{k=1}^{d} \Pr\left(X_{(i,k)}-f^{S}_{(i,m)}
    \geqslant\varepsilon\right)
\leqslant
    \left(\frac{1}{\epsilon\cdot w}\cdot
    \left(\sum_{i'=1}^{n} f_{i'}\right)\right)^{d}.
\end{align}
\postproof \end{proof}

==> SIGMOD21/zyk/theorem_error.tex <==
\begin{theorem}[Variance Bound]
\label{theo:error}



Given a data stream $\mathcal{S}$, 
%
for any strategy $\mathcal{P}$ and any item $i$, 
%
let $\hat{f_i}$ be the unbiased estimation of $f_i$ given by \uf{}, 
%
then we have
%
\begin{align}
\label{form:loss}
    D\left(\hat{f_i}\right)
\leqslant
    \frac{1}{d\cdot (w-1)}
    \cdot
    \left(
    \sum_{i'=1}^{n} 
    f_{i'}^2
    \right).
\end{align}
%
Where $d$ and $w$ are parameters of the \bcs{}.


\end{theorem}




\preproof \begin{proof}
\label{prf:error}



We consider a process $\mathcal{R}$ of strategy $\mathcal{P}$ on data stream $\mathcal{S}$, 
%
and prove that the conditional variance $D\left(\hat{f_i}~|~\mathcal{R}\right)$ of any item $i$ satisfies the above bound.



Recalling the definition of $\hat{f_i}$ and $f^{S'}_{(i,m)}$ in Proof \ref{theo:unbias}, 
%
we have
%
\begin{align}
    \hat{f_i}
=
    \begin{aligned}
    f^{T}_{(i,m)}
    \\
    + \frac{1}{d}\cdot
    \left(\sum_{k=1}^{d}
    \left(X_{(i,k)} - \frac{1}{w-1} \cdot
    \left(\sum_{i'=1}^{n} f^{S}_{(i',m)} - X_{(i,k)}\right)
    \right)
    \right)
    \end{aligned}.
\end{align}
%
Since 
%
$f^{T}_{(i,m)}$ and $f^{S}_{i',m}$ are constants when $\mathcal{R}$ is determined, we have
%
\begin{align}
&
    D\left(\hat{f_i}~|~\mathcal{R}\right)
\notag\\
=&
    D\left(
    \begin{aligned}
    f^{T}_{(i,m)}
    \\
    +\frac{1}{d}\cdot
    \left(\sum_{k=1}^{d}
    \left(X_{(i,k)}-\frac{1}{w-1}\cdot
    \left(\sum_{i'=1}^{n} f^{S}_{(i',m)}-X_{(i,k)}\right)
    \right)
    \right)
    \end{aligned}
    ~|~\mathcal{R}\right)
\notag\\
=&
    D\left(\frac{1}{d}\cdot
    \left(\sum_{k=1}^{d}
    \frac{w}{w-1} \cdot X_{(i,k)}\right)
    ~|~\mathcal{R}\right)
\notag\\
=&
    \frac{1}{d^2}\cdot
    \left(\sum_{k=1}^{d}
    \left(
    \left(\frac{w}{w-1}\right)^2
    \cdot
    D\left(X_{(i,k)}~|~\mathcal{R}\right)
    \right)
    \right).
\end{align}
%
%
By expanding $X_{(i,k)}$ and considering the independence between $I_{(i,i',k)}$, we have
%
%
\begin{align}
    D\left(X_{(i,k)}~|~\mathcal{R}\right)
=&
    D\left(f^{S}_{(i,m)} + \sum_{i'=1,i'\ne i}^{n} 
    \left(I_{(i,i',k)} \cdot f^{S}_{(i',m)}\right)
    ~|~\mathcal{R}\right)
\notag\\
=&    
    \sum_{i'=1,i'\ne i}^{n} 
    \left(
    \left(f^{S}_{(i',m)}\right)^2 \cdot 
    D\left(I_{(i,i',k)}~|~\mathcal{R}\right)
    \right)
\notag\\
=&
    \frac{1}{w} \cdot
    \left(1-\frac{1}{w}\right) \cdot
    \left(\sum_{i'=1,i'\ne i}^{n} 
    \left(f^{S}_{(i',m)}\right)^2
    \right)
\notag\\
\leqslant&
    \frac{1}{w} \cdot
    \left(1-\frac{1}{w}\right) \cdot
    \left(\sum_{i'=1}^{n} 
    \left(f^{S}_{(i',m)}\right)^2
    \right).
\end{align}
%
%
In other words
\begin{align}
\label{form:tight}
&
    D\left(\hat{f_i}~|~\mathcal{R}\right)
\notag\\
\leqslant&
    \frac{1}{d^2} \cdot
    \left(\sum_{k=1}^{d}
    \left(
    \left(\frac{w}{w-1}\right)^2 \cdot
    \left(\frac{1}{w} \cdot
    \left(1-\frac{1}{w}\right) \cdot
    \left(\sum_{i'=1}^{n}\left(f^{S}_{(i',m)}\right)^2\right)
    \right)
    \right)
    \right)
\notag\\
=&
    \frac{1}{d\cdot (w-1)} \cdot
    \left(\sum_{i'=1}^{n}\left(f^{S}_{(i',m)}\right)^2\right).
\end{align}
%
According to Lemma~\ref{lem:mono}, we have
%
\begin{align}
    D\left(\hat{f_i}~|~\mathcal{R}\right) \leqslant
    \frac{1}{d\cdot (w-1)} \cdot
    \left(\sum_{i'=1}^{n} f_{i'}^2\right).
\end{align}


In Proof \ref{theo:unbias}, we get 
%
%
\begin{align}
    E\left(\hat{f_i}~|~\mathcal{R}\right) =
    E\left(\hat{f_i}\right) = f_i.
\end{align}
%
%
Therefore, by using the law of total expectation, we can get that for strategy $\mathcal{P}$, there is
%
%
\begin{align}
    D\left(\hat{f_i}\right)
=&
    E\left(\left(\hat{f_i}-f_i\right)^2\right)
\notag\\
=&
    E_{\mathcal{R}\sim\mathcal{P}(\mathcal{S})}\left(
    E\left(
    \left(\hat{f_i}-f_i\right)^2~|~\mathcal{R}\right)
    \right)
\notag\\
=&
    E_{\mathcal{R}\sim\mathcal{P}(\mathcal{S})}
    \left(D\left(\hat{f_i}~|~\mathcal{R}\right)\right)
\notag\\
\leqslant&
    \frac{1}{d\cdot (w-1)} \cdot
    \left(\sum_{i'=1}^{n} f_{i'}^2\right).
\end{align}


\end{proof} \postproof

==> SIGMOD21/zyk/theorem_freezing.tex <==
\begin{theorem}[Unbiasedness of Error Freezing]
\label{theo:freezing_unbias}


Given a data stream $\mathcal{S}$, let $t_i$ be the time when item $i$ is recorded by \bp{}.
%
If item $i$ is not recorded, let $t_i=m$.
%
Let $\tilde{f_i}=f^{T}_{(i,m)}+f^{S'}_{(i,t_i)}$ be an estimation of $f_i$ with error freezing given by UTF.
%
For any strategy $\mathcal{P}$ and any item $i$, there is
%
\begin{align}
    E\left(\tilde{f_i}\right) = f_i.
\end{align}

\end{theorem}


\preproof \begin{proof}


Following the idea in Proof~\ref{theo:unbias}, we only need to prove that for any process $\mathcal{R}$ of strategy $\mathcal{P}$, 
%
there is
%
\begin{align}
    E\left(f^{S'}_{(i,t_i)}~|~\mathcal{R}\right) =
    f^{S}_{(i,m)}.
\end{align}


When $j>t_i$, the occurrence of item $i$ will always be recorded in the top-$K$ part instead of the sketch part, so we have $f^{S}_{(i,j)}=f^{S}_{(i,j-1)}$, and thus $f^{S}_{(i,t_i)}=f^{S}_{(i,m)}$.


Let the random variable $X_{(i,j,k)}$ be the value of the $h(i)$-th counter in the $k$-th array in the sketch part at time $j$, thus we have
%
\begin{align}
    f^{S'}_{(i,t_i)} = \frac{1}{d}\cdot
    \left(\sum_{k=1}^{d}
    \left(X_{(i,t_i,k)} - \frac{1}{w-1}\cdot
    \left(\sum_{i'=1}^{n} f^{S}_{(i',t_i)} - X_{(i,t_i,k)}\right)
    \right)
    \right).
\end{align}
%
According to the rules of the sketch part, we have
%
\begin{align}
&
    E\left(f^{(3')}_{(i,t_i)}~|~\mathcal{R}\right)
\notag\\
=&
    E\left(\frac{1}{d}\cdot
    \left(\sum_{k=1}^{d}
    \left(X_{(i,t_i,k)} - \frac{1}{w-1}\cdot
    \left(\sum_{i'=1}^{n} f^{S}_{(i',t_i)} - X_{(i,t_i,k)}\right)
    \right)
    \right)~|~\mathcal{R}\right)
\notag\\
=&
    \frac{1}{d} \cdot
    \left(\sum_{k=1}^{d}
    \left(\frac{w}{w-1} \cdot
    E\left(X_{(i,t_i,k)}~|~\mathcal{R}\right) - \frac{1}{w-1} \cdot
    \left(\sum_{i'=1}^{n} f^{S}_{(i',t_i)}\right)
    \right)
    \right)
\notag\\
=&
\begin{aligned}
    \frac{1}{d} \cdot
    \left(\sum_{k=1}^{d}
    \left(\frac{w}{w-1} \cdot
    E\left(f^{S}_{(i,t_i)} +
    \sum_{i'=1,i'\ne i}^{n} \left(I_{(i,i',k)} \cdot
    f^{S}_{(i',t_i)}\right)~|~\mathcal{R}
    \right)
    \right)
    \right)
    \\
    - \frac{1}{w-1} \cdot 
    \left(\sum_{i'=1}^{n} f^{S}_{(i',t_i)}\right)
\end{aligned}
\notag\\
=&
\begin{aligned}
    \frac{1}{d} \cdot \frac{w}{w-1} \cdot
    \left(\sum_{k=1}^{d}
    \left(\sum_{i'=1,i'\ne i}^{n}
    \left(
    f^{S}_{(i',t_i)} \cdot E\left(I_{(i,i',k)}~|~\mathcal{R}\right)
    \right)
    \right)
    \right)
    \\
    +\frac{w}{w-1} \cdot f^{S}_{(i,t_i)} - \frac{1}{w-1} \cdot
    \left(\sum_{i'=1}^{n} f^{S}_{(i',t_i)}\right)
\end{aligned}
\notag\\
=&
    \frac{1}{w-1} \cdot
    \left(\sum_{i'=1,i'\ne i}^{n} f^{S}_{(i',t_i)}\right)
    + \frac{w}{w-1} \cdot f^{S}_{(i,t_i)} - \frac{1}{w-1} \cdot
    \left(\sum_{i'=1}^{n} f^{S}_{(i',t_i)}\right)
\notag\\
=&
    f^{S}_{(i,t_i)}
\end{align}
%
%
Which means we have
%
%
\begin{align}
    E\left(\tilde{f_i}~|~\mathcal{R}\right)
=&
    f^{T}_{(i,m)}+
    E\left(f^{S'}_{(i,t_i)}~|~\mathcal{R}\right)
\notag\\
=&
    f^{T}_{(i,m)} + f^{S}_{(i,t_i)}
\notag\\
=&
    f^{T}_{(i,m)} + f^{S}_{(i,m)} = f_i.
\end{align}
%
%
Using the law of total expectation, we have
%
\begin{align}
    E\left(\tilde{f_i}\right) =
    E_{\mathcal{R}\sim\mathcal{P}(\mathcal{S})}
    \left(E\left(\tilde{f_i}~|~\mathcal{R}\right)\right)
    = f_i.
\end{align}


\end{proof} \postproof



\begin{theorem}[Variance Bound of Error Freezing]
\label{theo:freezing_bound}


Given a data stream $\mathcal{S}$, for any strategy $\mathcal{P}$ and any item $i$, we have
%
\begin{align}
    D\left(\tilde{f_i}\right) \leqslant D\left(\hat{f_i}\right).
\end{align}
\end{theorem}



\preproof \begin{proof}


We compare the conditional variance of $\hat{f_i}$ and $\tilde{f_i}$.
%
Given a process $\mathcal{R}$ of strategy $\mathcal{P}$, following the idea in the Proof~\ref{theo:error}, we have
%
\begin{align}
    D\left(
    \tilde{f_i}~|~\mathcal{R}
    \right)
=&
    \frac{1}{d^2}\cdot
    \left(
    \sum_{k=1}^{d}
    \left(
    \left(
    \frac{w}{w-1}
    \right)^2
    \cdot
    D\left(
    X_{(i,t_i, k)}
    ~|~\mathcal{R}\right)
    \right)
    \right)
\notag\\
=&
    \frac{1}{d\cdot (w-1)}
    \cdot
    \left(
    \sum_{i'=1,i'\ne i}^{n} 
    \left(f^{(3)}_{(i',t_i)}\right)^2
    \right).
\end{align}
%
%
According to Lemma~\ref{lem:mono}, we have
%
\begin{align}
    f^{(3)}_{(i',t_i)}\leqslant f^{(3)}_{(i',m)}.
\end{align}
%
In other words,
%
\begin{align}
    D\left(
    \tilde{f_i}~|~\mathcal{R}
    \right)
=&
    \frac{1}{d\cdot (w-1)}
    \cdot
    \left(
    \sum_{i'=1,i'\ne i}^{n} 
    \left(f^{(3)}_{(i',t_i)}\right)^2
    \right)
\notag\\
\leqslant&
    \frac{1}{d\cdot (w-1)}
    \cdot
    \left(
    \sum_{i'=1,i'\ne i}^{n} 
    \left(f^{(3)}_{(i',m)}\right)^2
    \right)
=
    D\left(
    \hat{f_i}~|~\mathcal{R}
    \right)
\end{align}
%
Using the law of total expectation, we have
%
\begin{align}
    D\left(\hat{f_i}\right)
=&
    E_{\mathcal{R}\sim\mathcal{P}(\mathcal{S})}\left(
    D\left(
    \tilde{f_i}
    ~|~\mathcal{R}\right)
    \right)
\notag\\
\leqslant&
    E_{\mathcal{R}\sim\mathcal{P}(\mathcal{S})}\left(
    D\left(
    \hat{f_i}
    ~|~\mathcal{R}\right)
    \right)
=
    D\left(\tilde{f_i}\right).
\end{align}

\end{proof} \postproof

==> SIGMOD21/zyk/theorem_ineq.tex <==
\begin{theorem}[overestimations and underestimations]
\label{theo:ineq}


Given a data stream $\mathcal{S}$, 
%
for any strategy $\mathcal{P}$, 
%
let 
%
\begin{align}
    \underline{f_i} &= f^{T}_{(i,m)}.
    \notag\\
    \overline{f_i} &= f^{T}_{(i,m)} +
    \left(\min_{k=1}^{d} X_{(i,k)} \right).
\end{align}
%

Where $X_{(i,k)}$ is defined in Proof~\ref{theo:unbias}.
%
Then for any item $i$, there is
%
\begin{align}
    \underline{f_i} \leqslant f_i \leqslant \overline{f_i}.
\end{align}


\end{theorem}

\preproof \begin{proof}
\label{prf:ineq}




Given a data stream $\mathcal{S}$ and a strategy $\mathcal{P}$, according to Lemma \ref{lem:iden}, we know that for any process $\mathcal{R}$ and item $i$, there is
%
%
\begin{align}
    f^{T}_{(i,m)} + f^{S}_{(i,m)} = f_i.
\end{align}
%
According to Lemma~\ref{lem:mono}, we know that $f^{S}_{(i,m)}\geqslant 0$.
%
Then we can get 
%
\begin{align}
    \underline{f_i} = f^{S}_{(i,m)} \leqslant f^{S}_{(i,m)}+f^{T}_{(i,m)} = f_i.
\end{align}
%
Because of the arbitrariness of process $\mathcal{R}$, we can get $\underline{f_i}\leqslant f_i$ always holds.


By recalling the $X_{(i,k)}$ defined in Proof \ref{theo:unbias}, we have
%
\begin{align}
    X_{(i,k)} = f^{S}_{(i,m)} + \sum_{i'=1,i'\ne i}^{n}
    \left(f^{S}_{(i',m)} \cdot I_{(i,i',k)} \right)
    \geqslant f^{S}_{(i,m)}.
\end{align}
%
Taking the above inequality into the definition of $\overline{f_i}$, we can get
%
\begin{align}
    \overline{f_i} = f^{T}_{(i,m)} +
    \left(\min_{k=1}^{d} X_{(i,k)}\right) \geqslant
    f^{T}_{(i,m)} + f^{S}_{(i,m)} = f_i.
\end{align}
%S
That is, $\overline{f_i}\geqslant f_i$ always holds.
%
To sum up, for any strategy $\mathcal{P}$, $\underline{f_i}\leqslant f_i\leqslant \overline{f_i}$ always holds.

\end{proof} \postproof

==> SIGMOD21/zyk/theorem_unbiased.tex <==

\begin{theorem}[Unbiasedness]
\label{theo:unbias}



Given a data stream $\mathcal{S}$.
%
Let $f^{S'}_{(i,j)}$ $\left(C_{unbiased}\right)$ be the estimate of $f^{S}_{(i,j)}$ given by the sketch part at time $j$.
%
Let $\hat{f_{i}}=f^{T}_{(i,m)}+f^{S'}_{(i,m)}$ be the estimation of $f_{i}$ given by UTF.
%
For any strategy $\mathcal{P}$ of finding top-$K$ items and any item $i$, there is
%
\begin{align}
E\left(\hat{f_{i}} \right)=f_i.
\end{align}
\end{theorem}

\preproof \begin{proof}
\label{prf:unbias}



We first prove that for any process $\mathcal{R}$ of strategy $\mathcal{P}$, 
%
the estimation $\hat{f_i}$ of any item $i$ given by process $\mathcal{R}$ is unbiased, \ie, 
%
\begin{align}
    E\left(\hat{f_{i}}~|~\mathcal{R}\right)=f_i.
\end{align}


We have the estimation $\hat{f_{i}} = f^{T}_{(i,m)}-+f^{S'}_{(i,m)}$, the frequency $f_i=f_{(i,m)}$, and according to Lemma \ref{lem:iden} we have
%
\begin{align}
f^{T}_{(i,m)}+f^{S}_{(i,m)} = f_{(i,m)}.
\end{align}
%
Since $f^{T}_{(i,m)}$ is determined by process $\mathcal{R}$, if we want to prove $E\left(\hat{f_{i}}~|~\mathcal{R}\right)=f_i$, \ie, 
%
\begin{align}
    E\left(f^{T}_{(i,m)}+f^{S'}_{(i,m)}~|~\mathcal{R}\right)
    =
    f^{T}_{(i,m)}+f^{(S)}_{(i,m)},
\end{align}
%
we only need to prove
%
\begin{align}
    E\left(f^{S'}_{(i,m)}~|~\mathcal{R}\right)
    =f^{S}_{(i,m)}, 
\end{align}
%
as described below.




We use a CMM~\cite{CMM} sketch as sketch part. 
%
Specifically, assume that the sketch part uses $d$ counter arrays, each with its length $w$ and a hash function $h_k(\cdot)$.
%
$h_k(\cdot)$ maps each item $i$ to one of the $w$ counters uniformly at random.


We define some useful random variables.
%
Let the indicator random variable $I_{(i,i',k)}$ indicates whether $h_k(i)$ and $h_k(i')$ are equal, thus we have
%
\begin{align}
    \Pr\left(I_{(i,i',k)}=1\right)=\frac{1}{w}.
\end{align}
%
Let the random variable $X_{(i,k)}$ be the value of the $h_k(i)$-th counter in the $k$-th array, 
%
thus we have
%
\begin{align}
    f^{S'}_{(i,m)}=
    \frac{1}{d}\cdot
    \left(\sum_{k=1}^{d}
    \left(X_{(i,k)}-\frac{1}{w-1}\cdot
    \left(\sum_{i'=1}^{n} f^{S}_{(i',m)}-X_{(i,k)}\right)
    \right)
    \right).
\end{align}

Next, we analyze the conditional expectation of $f^{S'}_{(i,m)}$.
%
According to the rules of the CMM, we have
%
\begin{align}
    X_{(i,k)}=f^{S}_{(i,m)} + \sum_{i'=1,i'\ne i}^{n}
    \left(I_{(i,i',k)}\cdot f^{S}_{(i',m)}\right).
\end{align}
\label{form:rv}
%
We can obtain the conditional expectation of $X_{i,k}$, namely
%
\begin{align}
    E\left(X_{(i,k)}~|~\mathcal{R}\right)
=&
    E\left(f^{S}_{(i,m)} + \sum_{i'=1,i'\ne i}^{n} 
    \left(I_{(i,i',k)}\cdot f^{S}_{(i',m)}\right)
    ~|~\mathcal{R}\right)
\notag\\
=&
    f^{S}_{(i,m)} + \sum_{i'=1,i'\ne i}^{n}
    \left(f^{S}_{(i',m)} \cdot 
    E\left(I_{(i,i',k)}~|~\mathcal{R}\right)
    \right)
\notag\\
=& 
    f^{S}_{(i,m)} + \sum_{i'=1,i'\ne i}^{n}
    \left(f^{S}_{(i',m)} \cdot \frac{1}{w}\right)
\notag\\
=&
    f^{(3)}_{(i,m)} + \frac{1}{w}\cdot
    \left(\sum_{i'=1,i'\ne i}^{n} f^{S}_{(i',m)}\right).
\end{align}
%
%
Using the linear property of expectation again, we can get
%
\begin{align}
&
    E\left(f^{S'}_{(i,m)}~|~\mathcal{R}\right)
\notag\\
=&
    E\left(\frac{1}{d}\cdot
    \left(\sum_{k=1}^{d}
    \left(X_{(i,k)} - \frac{1}{w-1}\cdot
    \left(\sum_{i'=1}^{n} f^{S}_{(i',m)} - X_{(i,k)}\right)
    \right)
    \right)
    ~|~\mathcal{R}\right)
\notag\\
=&
    \frac{1}{d}\cdot
    \left(\sum_{k=1}^{d}
    \left(\frac{w}{w-1} \cdot
    E\left(X_{(i,k)}~|~\mathcal{R}\right) -
    \frac{1}{w-1}\cdot
    \left(\sum_{i'=1}^{n} f^{S}_{(i',m)}\right)
    \right)
    \right)
\notag\\
=&
    \frac{1}{d}\cdot
    \left(\sum_{k=1}^{d}
    \left(
    \begin{aligned}
    \frac{w}{w-1} \cdot
    \left(
    f^{S}_{(i,m)} + \frac{1}{w}\cdot
    \left(\sum_{i'=1,i'\ne i}^{n} f^{S}_{(i',m)}\right)
    \right)
    \notag\\
    -\frac{1}{w-1}\cdot
    \left(\sum_{i'=1}^{n} f^{S}_{(i',m)}\right)
    \end{aligned}
    \right)
    \right)
\notag\\
=&
    \frac{1}{d}\cdot
    \left(\sum_{k=1}^{d}
    \left(
    \frac{w}{w-1} \cdot f^{S}_{(i,m)} -
    \frac{1}{w-1} \cdot f^{S}_{(i,m)}
    \right)
    \right)
=
    f^{S}_{(i,m)}.
\end{align}

To sum up, 
%
we get that for any process $\mathcal{R}$,
%
$E\left(\hat{f_i}~|~\mathcal{R}\right)=f_i$ holds.
%
%
By using the law of total expectation, 
%
we get that for any strategy $\mathcal{P}$, there is
%
%
\begin{align}
    E\left(\hat{f_i}\right)
=&
    E_{\mathcal{R}\sim\mathcal{P}(\mathcal{S})}
    \left(E\left(\hat{f_i}~|~\mathcal{R}\right)\right)
\notag\\
=&
    \sum_{\mathcal{R}\sim\mathcal{P}(\mathcal{S})}
    \left(
    E\left(\hat{f_i}~|~\mathcal{R}\right) \cdot
    \Pr\left(\mathcal{R}\right)
    \right)
\notag\\
=&
    f_i \cdot
    \left(
    \sum_{\mathcal{R}\sim\mathcal{P}(\mathcal{S})}
    \Pr\left(\mathcal{R}\right)
    \right)
=
    f_i.
\end{align}

\end{proof} \postproof






\begin{theorem}[Conditional Unbiasedness]
\label{theo:cond_unbias}



Given a data stream $\mathcal{S}$.
%
For any strategy $\mathcal{P}$ and any item $i$, let $\mathcal{K}_i$ be the event that item $i$ is reported as a top-$K$ item,
%
there is
%
%
\begin{align}
E\left(\hat{f_{i}}~|~\mathcal{K}_i\right)=f_i.
\end{align}


\end{theorem}




\preproof \begin{proof}
\label{prf:cond_unbias}


The occurrence of event $\mathcal{K}_i$ depends entirely on process $\mathcal{R}$.
%
Thus for any process $\mathcal{R}\sim\mathcal{P}(\mathcal{S})$, we have either $\mathcal{R}\subset\mathcal{K}_i$ (\ie, item $i$ is reported as a top-$K$ item in process $\mathcal{R}$) or $\mathcal{R}\subset\overline{\mathcal{K}_i}$ (\ie, item $i$ is not reported as a top-$K$ item in process $\mathcal{R}$). 
%
By using the law of total expectation again, we have
%
%
\begin{align}
    E\left(\hat{f_i}~|~\mathcal{T}_i\right)
=&
    E\left(
    E\left(\hat{f_i}~|~\mathcal{R},\mathcal{T}_i\right)
    ~|~\mathcal{T}_i\right)
\notag\\
=&
    \sum_{\mathcal{R}\subset\mathcal{T}_i}
    \left(
    E\left(\hat{f_i}~|~\mathcal{R},\mathcal{T}_i\right) \cdot
    \Pr\left(\mathcal{R}~|~\mathcal{T}_i\right)
    \right)
\notag\\
=&
    \sum_{\mathcal{R}\subset\mathcal{T}_i}
    \left(
    E\left(\hat{f_i}~|~\mathcal{R}\right)\cdot
    \Pr\left(\mathcal{R}~|~\mathcal{T}_i\right)
    \right)
\notag\\
=&
    f_i\cdot
    \left(
    \sum_{\mathcal{R}\subset\mathcal{T}_i}
    \Pr\left(\mathcal{R}~|~\mathcal{T}_i\right)
    \right)
=
    f_i.
\end{align}

\end{proof} \postproof

==> TODO.tex <==
% 1. 修改关于CM bound的说法
% 2. 1.1关于weighted的方法在1.2简述，在实验部分描述
% 3. 用disjoint data streams替换distributed data streams
% 4. 查看uinbiased的使用
% 5. definition改成theorem的形式并加以描述
% 6. 把top-k-fairness改成更加通用的描述
% 7. 2.2改成unbiasedness v.s. top-k-fairness，2.3讲CMM
% 8. 证明lemma 4.1，把lemma 4.2放到freeeze的部分
% 9. 数学部分证明前说明是证明的hot panning版本

==> tex/empty.tex <==


% Filters aim to determine whether an item $e\in \mathcal{U}$ belongs to a subset $\mathcal{S}\subset \mathcal{U}$ within (expected) constant time. They have two main operations: construction and query. If a filter can also dynamically insert new items, it is called a dynamic filter. Typically, the filters have only one-sided error, which means they must say ``yes'' if $e\in \mathcal{S}$ and may produce a small false positive rate $\epsilon$ if $e\notin \mathcal{S}$. For convenience, we refer to the items in $\mathcal{S}$ as ``positive'' items and those in $\mathcal{U}\backslash\mathcal{S}$ as ``negative'' items, $|\mathcal{S}|:=n\gg1, |\mathcal{U}\backslash\mathcal{S}|:=\lambda n$\footnote{In this paper, we use $n$ and $\lambda n$ to represent $|\mathcal{S}|$ and $|\mathcal{U}\backslash\mathcal{S}|$, respectively. However, to simplify notation, we avoid using $(\lambda+1)n$ to represent $|\mathcal{U}|$.}.

%Given a universe $\mathcal{U}$ and subset $\mathcal{S}\in \mathcal{U}$, the membership filters aim to answer whether an item $e\in \mathcal{U}$ is in $\mathcal{S}$ within (expected) constant time. The basic operation of a filter is construction and query. If it also supports insertion of new items, the filter is called a dynamic filter. Typically, the filters only satisfy one-side error: it must say yes if $e\in \mathcal{S}$, and may make mistake with a small false positive rate $\epsilon$ if $e\notin \mathcal{S}$.  %In this paper, we assume every item has independent (unrelated) ID and equal query probability.
%For convenience, we call items in $\mathcal{S}$ as positive items and items in $\mathcal{U}\backslash\mathcal{S}$ as false items, $|\mathcal{S}|:=n\gg1, |\mathcal{U}\backslash\mathcal{S}|:=\lambda n$\footnote{In this paper, we use $n$ and $\lambda n$ to represent $|\mathcal{S}|$ and $|\mathcal{U}\backslash\mathcal{S}|$. But we tend to avoid using $(\lambda+1)n$ to represent $|\mathcal{U}|$ for simplicity concerns.}.

Although there are various Bloom Filter variants weighing on space, throughput and simplicity \cite{cohen2003spectral, kirsch2006less,dutta2013streaming}, we can categorize them into three schemes.
%
The \textbf{first} scheme assumes that $\lambda \gg 1$, and thus only encodes positive items (e.g., Bloom Filter \cite{bloom1970space}, Cuckoo Filter \cite{fan2014cuckoo}, and Binary Fuse Filter \cite{graf2022binary}). For instance, the Binary Fuse Filter encodes $\alpha$-bit fingerprints for all positive items within $Cn\alpha =Cn\log1/\epsilon$ bits\footnote{$\log$ is base 2, $\ln$ is base $e\approx2.718$ throughout this paper.}, where $C$ can be any constant greater than 1. While the Binary Fuse Filter always recognizes positive items, it may have a false positive rate $\epsilon=1/2^\alpha$ due to fingerprint collisions. In fact, $\log1/\epsilon$ bits per item is the space lower bound \cite{carter1978exact}.
%The first scheme assumes $\lambda \gg 1$, and thus only encodes positive items (e.g. Bloom Filter \cite{bloom1970space}, Cuckoo Filter \cite{fan2014cuckoo}, and Binary Fuse Filter \cite{graf2022binary}). For instance, the Binary Fuse Filter encodes $\alpha$-bit fingerprints for all positive items within $Cn\alpha =Cn\log1/\epsilon$ space in bits\footnote{$\log$ is base 2 throughout this paper.}, where $C$ can be any constant greater than 1. Binary Fuse Filter always recognizes positive item, but may have false positive rate $\epsilon=1/2^\alpha$ due to fingerprint collisions. In fact, $\log1/\epsilon$ bits per item is the space lower bound \cite{carter1978exact}.
%
The \textbf{second} scheme constructs a perfect hash table for all items and recognizes them with no error (e.g., Bloomier Filter \cite{chazelle2004bloomier,charles2008bloomier}, Othello Hashing \cite{yu2018memory}, and Coloring Embedder \cite{tong2019coloring}). For instance, the Bloomier Filter encodes 1-bit fingerprints for all $|\mathcal{U}|$ items within $C|\mathcal{U}|$ bits.

In this paper, all other filters fall under the \textbf{third} scheme, among which we are particularly interested in combined filters. In recent years, researchers have found that %creatively introduce machine learning methodology \cite{kraska2018case} to construct Learned Bloom Filters \cite{mitzenmacher2018model,liu2020stable,dai2020adaptive}. 
combining learned oracles and/or pre-filters with current filter structures can significantly improve accuracy \cite{mitzenmacher2018model,liu2020stable,dai2020adaptive,reviriego2021approximate}. This is partly because a learned structure may capture the relationships among item IDs, but is also partly because different elementary data structures have different properties that can work better in combination. In this paper, we assume that item IDs are independent, excluding the interference of the first reason. We ask, \textbf{what is a good combination}? \textit{Can we develop a theory to factorize a membership query problem into several sub-problems, solve them independently using sub-structures, and then combine the sub-structures to achieve optimal performance?} These questions motivate this work.

%\subsection{This Work}



To address these questions, we first generalize the space lower bound of approximate (i.e. the case where $\lambda \to +\infty$) and exact (i.e. the case where $\epsilon=0$) membership query problems \cite{carter1978exact} to arbitrary $(\epsilon, \lambda)$ pair (i.e. $\forall \epsilon\in [0,1], \lambda \in \mathbb{R}^+$). We demonstrate that a filter must use at least 
$$n\mathcal{L}^*_{\epsilon,\lambda}+o(n):=n(\lambda+1)H\left(\frac{1}{\lambda+1}\right)-n(\epsilon\lambda+1)H\left(\frac{1}{\epsilon\lambda+1}\right)+o(n)$$
bits to achieve a false positive rate of $\epsilon$, where $H(p):=-p\log p-(1-p)\log(1-p)$ represents Shannon's entropy (\textbf{Theorem \ref{algo::lower bound}}). 



Next, inspired by the form of $\mathcal{L}^*_{\epsilon,\lambda}$ and the identity
$$\mathcal{L}^*_{\epsilon_1\epsilon_2,\lambda}= \mathcal{L}^*_{\epsilon_1,\lambda}+\mathcal{L}^*_{\epsilon_2,\epsilon_1\lambda},$$
we introduce the \textbf{chain rule} to factorize one membership query problem into multiple sub-problems without information loss (ignore $o(n)$, \textbf{Theorem \ref{thm::chain rule}}). Specifically, we show that a membership query filter with $n$ positive items, $\lambda n$ negative items, and false positive rate $\epsilon_1 \epsilon_2$ can be factorized into two parts: The first part is a filter for $n$ positive items and $\lambda n$ negative items with false positive rate $\epsilon_1$, and the second part is a filter for $n$ positive items and $\epsilon_1\lambda n$ negative items with false positive rate $\epsilon_2$, denoted as
$$\langle\epsilon_1\epsilon_2,\lambda\rangle \rightarrow \langle\epsilon_1,\lambda\rangle\circ \langle\epsilon_2,\epsilon_1\lambda\rangle.$$
We call this factorization theorem as the chain rule due to its transitivity. The chain rule is intuitive once we observe that the expected number of false positive items of the first filter is $\epsilon_1\lambda n$. But it is also nontrivial because the factorization process is \textbf{lossless}: if we can construct two space-optimal sub-filters, we can combine them to create a space-optimal parent-filter and subsequently a space optimal grandparent-filter. In other words, combining filters according to the chain rule results in space overhead only from its elementary filters, and the factorization process does not incur any systematical space overhead at all.

Finally, based on the chain rule, we combine the first and the second scheme filters to design our \algoname{} (\textbf{Algorithm \ref{algo::construct}}), which significantly outperforms any first or second scheme filter. \algoname{} requires only 
$$Cn\left(\lfloor\log \lambda\rfloor+1+\frac{\lambda}{2^{\lfloor\log \lambda\rfloor}}\right)\in [Cn \log(2e\lambda\ln2), Cn\log 4\lambda]$$
\begin{wrapfigure}{l}{2.5cm}\vspace{-0.4in}
\includegraphics[width=0.2\textwidth]{tex/fig/fourcurves.pdf}\label{pic::fourcurves}\vspace{-0.8cm}
\end{wrapfigure} bits to exactly classify $n$ positive items and $\lambda n$ negative items, which is less than 1.11 times the space infimum $n\mathcal{L}^*_{0,\lambda}$ (ignore $o(n)$). In contrast, using only the first (resp. the second) scheme filter necessitates $O(n\log \lambda n)$ (resp. $C|\mathcal{U}|$) space. We display the trend when $\lambda=16$ and $C\to 1$ in the left figure. Another important feature of \algoname{} is its \textbf{simplicity}: We prove that if we restrict the elementary filters to Bloomier Filters and combine them with the operator ``\&'', the space-optimal solution consists of only two filters (\textbf{Theorem \ref{algo::optimality}})\footnote{For elementary filters, we provide the optimal space cost in \textbf{Theorem \ref{algo::limit}}.}. Moreover, we discover that the chain rule offers new insights for designing novel membership query algorithms. If we replace the operator with others like ``$\&\sim$'', we can derive new \algoname{} variants eliminating additional construction space (\textbf{Theorem \ref{algo::variant}}), at the expense of 
modest construction time ($O(|\mathcal{U}|\log \log n)$ vs $O(|\mathcal{U}|)$). We believe that \algoname{} and its variants can be widely applied in data compressing (\textbf{Section \ref{perf::compact truth table}, \ref{perf::randomized huffman coding}}), classifying (\textbf{Section \ref{perf::sah}}), filtering (\textbf{Section \ref{perf::lsmtree}}), and more applications. 


%Specially, we think skipping \textbf{Section \ref{algo::warm up}} and \textbf{\ref{algo::general}} will not significantly impede the comprehension of this paper.

\subsection{Key Contributions}

In general, the main organization logic of this paper is
\begin{equation*}
\begin{split}
&``\textbf{(\S\textbf{\ref{algo::lower bound})} Theoretical lower bound} \xrightarrow[\textbf{\S\ref{algo::chain rule}}]{\textbf{derive}} \textbf{Chain rule theory}  \\
&\xrightarrow[\textbf{\S\ref{algo::key design}-\ref{algo::framework}}]{\textbf{design}}\textbf{\algoname{}} \xrightarrow[\S\textbf{\ref{perf}}]{\textbf{deploy}} \textbf{Potential applications''}.
\end{split}
\end{equation*}
Our key contributions are:

\noindent$\bullet$ We present the space lower bound for membership query with arbitrary false positive rate $\epsilon$ and false-positive ratio $\lambda$. From this, we derive a factorization theorem, namely the chain rule, which allows us to factorize one membership query problem into several sub-problems without information loss (ignore $o(n)$). 

\noindent$\bullet$ Based on the chain rule, we propose \algoname{} framework which combines elementary membership filters to promote space efficiency. We evaluate its performance for data compressing, classifying and filtering applications. Both theoretical and experimental results show that \algoname{} performs well: (1) it requires only 26\% additional space over the theoretical lower bound to encode an implicit static dictionary, (2) it requires only 0.22 additional bit per item over the theoretical lower bound for lossless data compression, (3) it reduces up to 31\% external memory access for Cuckoo Hashing \cite{fan2014cuckoo}, and (4) it reduces up to 36\% \texttt{P99} tail point query latency in RocksDB database \cite{dong2021rocksdb}. We will further introduce these applications in \textbf{Section \ref{perf}}. Our open source code is on GitHub \cite{ChainedFilterURL}.

==> tex/letter.tex <==
\section*{\centerline{Cover Letter}}

\balance

\begin{multicols}{2}

We sincerely thank the reviewers and the chairs, and we try our best to update the paper according to professional and helpful comments.
%
We use different colors in the paper to emphasize \revise{major updates} and \update{minor updates}.
%
Our updates on the issues highlighted in the Meta-Review are summarized below, and some minor updates on writing style and format are shown in the paper.
%
In response, we use hyperlinks [\revise{link}] that can jump to the location of the updated content in the paper.

\vspace{0.2cm}\bbb{\textit{\large Conceptual clarifications about fairness and bias.}}\vspace{0.2cm}

\bbb{R1-O1}: The differences between biased and unbiased algorithms.

\bbb{Response:}
%
In Section \ref{sec:related:unbias}, we introduce some well-known biased and unbiased algorithms [\hyperlink{link:ub_algo}{\revise{link}}], and formally define the concept of \textit{unbiased algorithm} through Definition \ref{def:unbias} [\hyperlink{link:ub_def}{\revise{link}}].
%
\vspace{0.12cm}

\bbb{R2-O1}: The difference and relation between fairness and unbiasedness.

\bbb{Response:}
%
In section \ref{sec:related:unbias}, we take USS [\hyperlink{link:diff_uss}{\revise{link}}] and WavingSketch [\hyperlink{link:diff_waving}{\revise{link}}] as examples to discuss the relationship between \textit{unbiasedness} and \textit{\fairness{}} in detail.
%
\vspace{0.12cm}

\bbb{R3-O1}: The formal definition of the fairness.

\bbb{Response:}
%
In Section \ref{related::pre}, we formally define \fairness{} [\hyperlink{link:def_fair}{\revise{link}}] and discuss the existing work on fairness and equality in the field of machine learning and recommendation system [\hyperlink{link:disc_fair}{\revise{link}}].
%
\vspace{0.12cm}

\bbb{R3-O2}: The terminology used in the paper.

\bbb{Response:}
%
We replace \textit{fairness} with \textit{\fairness}.
%
\vspace{0.12cm}

\vspace{0.2cm}\bbb{\textit{\large Presentation issues.}}\vspace{0.2cm}

\bbb{R1-O2}: The scenario of distributed data streams.

\bbb{Response:}
%
We replace \textit{distributed data streams} with more formal \textit{disjoint data streams}, and give a formal definition in Section \ref{related::pre} [\hyperlink{link:def_dis}{\revise{link}}].
%
\vspace{0.12cm}

\bbb{R1-O3}: The presentation of the results in Section 5.4.

\bbb{Response:}
%
We adjust Section \ref{sec:global_topk_imbalanced} to four subsections.
%
These subsections 1) describe the experimental settings, 2) show the \fairness{} or \unfairness{} of different algorithms and the impact of \fairness{} on performance, 3) show the impact of \fairness{} on different data streams, and 4) compare our algorithm with the other two baseline algorithms.
%
\vspace{0.12cm}

\bbb{R2-O4}: The formal definition of the problem.

\bbb{Response:}
%
In Section \ref{related::pre}, we give the formal definitions of \textit{disjoint data streams} [\hyperlink{link:def_dis}{\revise{link}}] and \textit{global top-$K$ items} [\hyperlink{link:def_topk}{\revise{link}}], and describe the general process of finding global top-$K$ items [\hyperlink{link:disc_topk}{\revise{link}}].
%
\vspace{0.12cm}


\bbb{R2-O5.1}: The distributed stream setting.

\bbb{Response:}
%
We replace \textit{distributed data streams} with more formal \textit{disjoint data streams}, and give a formal definition in Section \ref{related::pre} [\hyperlink{link:def_dis}{\revise{link}}].
%
\vspace{0.12cm}

\bbb{R2-O5.2}: The notion of double-anonymity.

\bbb{Response:}
%
We move the formal definition of \textit{double-anonymity} [\hyperlink{link:def_da}{\revise{link}}] and the proof that double-anonymity is a sufficient condition of \fairness{} [\hyperlink{link:proof_da}{\revise{link}}] to Section \ref{algo::dou}.
%
\vspace{0.12cm}

\bbb{R2-O8}: The technical depth and novelty of the paper.

\bbb{Response:}
%
We give the formal definition of the problem in Section \ref{related::pre} [\hyperlink{link:def_topk}{\revise{link}}], and emphasize the importance of \textit{defining \fairness{}} [\hyperlink{link:emp_fair}{\revise{link}}] and \textit{introducing two optimizations to the basic version} [\hyperlink{link:emp_opt}{\revise{link}}] in the introduction section.
%
\vspace{0.12cm}

\vspace{0.2cm}\bbb{\textit{\large A more reasonable baseline and the corresponding comparisons.}}\vspace{0.2cm}

\bbb{R2-O2}: The so-called "typical solution" indeed may be atypical.

\bbb{Response:}
%
We compare our algorithm with the weighted algorithms in Section \ref{sec:global_topk_imbalanced}.
%
These algorithms maintain data structures of different sizes for different data streams.
%
The experimental results (Figure \ref{fig:global_topk}) show our algorithm still outperforms the weighted algorithms  [\hyperlink{link:exp_cmp}{\revise{link}}].
%
We also discuss another manual algorithm, namely manually adjusting the frequency reported by different data streams, which is difficult in practice  [\hyperlink{link:disc_cmp}{\revise{link}}].
%
\vspace{0.12cm}

\bbb{R2-O7}: A straightforward baseline.

\bbb{Response:}
%
We compare our algorithm with the sampling algorithm in Section \ref{sec:global_topk_imbalanced}.
%
The experimental results (Table \ref{table:exp_sampling}) show the advantages of our algorithm, even in the case of lower transmission volume  [\hyperlink{link:exp_samp}{\revise{link}}].

\vspace{0.2cm}\bbb{\textit{\large Analytical comparison of replacement policies.}}\vspace{0.2cm}

\bbb{R2-O6}: The analytic comparison of four replacement policies.

\bbb{Response:}
%
We discuss the differences between four replacement policies based on the experimental results in Section 5.4.2 [\hyperlink{link:disc_rep_1}{\revise{link}}], Section 5.4.3 [\hyperlink{link:disc_rep_2}{\revise{link}}], and Section 5.5 [\hyperlink{link:disc_rep_3}{\revise{link}}], respectively, and show that our algorithm is general.
%
In Section \ref{sec:global_topk_imbalanced}, we show the degree of \unfairness{} of these four replacement policies, analyze how \unfairness{} affects their performance in the task of finding global top-$K$ items, and show that our Double-Anonymous sketch can indeed make them \fair{} (Figure \ref{fig:global_topk_1_2});
%
In Section \ref{subsec:Parameter Settings}, we show a more comprehensive performance comparison of Double-Anonymous sketch using different replacement policies (Figure \ref{fig:varying-params}).

\vspace{0.2cm}\bbb{\textit{\large Improvement on the experimental valuations.}}\vspace{0.2cm}

\bbb{R1-O4}: The statistical significance of the performance gaps.

\bbb{Response:}
%
In Section \ref{sec:global_topk_imbalanced}, we show the degree of \unfairness{} of different algorithms [\hyperlink{link:exp_rep_1}{\revise{link}}], and discuss how the degree of \unfairness{} impacts the overall performance of the algorithm (Figure \ref{fig:global_topk_1_2}) [\hyperlink{link:disc_rep_1}{\revise{link}}].
%
In general, the more significant the \unfairness{} is, the worse the overall performance of the algorithm will be.
%
In Section \ref{subsec:Parameter Settings}, we show a more comprehensive performance comparison of Double-Anonymous sketch using different configuration settings (Figure \ref{fig:varying-params}).
%
\vspace{0.12cm}

\bbb{R2-O3}: The definition of fairness.

\bbb{Response:}
%
In Section \ref{related::pre}, we modify the definition of \fairness{} to make it more general [\hyperlink{link:def_fair}{\revise{link}}].
%
The new definition could cover ratio-based fairness.
%
We discuss the existing work on fairness and equality in the field of machine learning and recommendation system [\hyperlink{link:disc_fair}{\revise{link}}].
%
In Section \ref{sec:global_topk_imbalanced}, we show the ratio of estimated frequency and real frequency reported by different algorithms [\hyperlink{link:exp_rep_1}{\revise{link}}].
%
The experimental results (Figure \ref{fig:global_topk_1_2}) show the \fairness{} of our algorithm and the \unfairness{} of other algorithms.
%
We discuss how \fairness{} impacts overall performance [\hyperlink{link:disc_rep_1}{\revise{link}}].

\end{multicols}
